A Geometric Framework for Adversarial Vulnerability in Machine Learning

This work starts with the intention of using mathematics to understand the intriguing vulnerability observed by ~\citet{szegedy2013} within artificial neural networks. Along the way, we will develop some novel tools with applications far outside of just the adversarial domain. We will do this while developing a rigorous mathematical framework to examine this problem. Our goal is to build out theory which can support increasingly sophisticated conjecture about adversarial attacks with a particular focus on the so called ``Dimpled Manifold Hypothesis'' by ~\citet{shamir2021dimpled}. Chapter one will cover the history and architecture of neural network architectures. Chapter two is focused on the background of adversarial vulnerability. Starting from the seminal paper by ~\citet{szegedy2013} we will develop the theory of adversarial perturbation and attack. Chapter three will build a theory of persistence that is related to Ricci Curvature, which can be used to measure properties of decision boundaries. We will use this foundation to make a conjecture relating adversarial attacks. Chapters four and five represent a sudden and wonderful digression that examines an intriguing related body of theory for spatial analysis of neural networks as approximations of kernel machines and becomes a novel theory for representing neural networks with bilinear maps. These heavily mathematical chapters will set up a framework and begin exploring applications of what may become a very important theoretical foundation for analyzing neural network learning with spatial and geometric information. We will conclude by setting up our new methods to address the conjecture from chapter 3 in continuing research.

==> Chapters/Chapter3a.tex <==
\chapter{Foundation for Study of Decision Boundaries} 
\label{Chapter3a}

A central issue when writing classifiers is mapping from continuous outputs or probabilities to discrete sets of classes. Frequently argmax type functions are used to accomplish this mapping. To discuss decision boundaries, we must precisely define argmax and some of its properties. 

In practice, argmax is not strictly a function, but rather a mapping from the set of outputs or activations from another model into the power set of a discrete set of classes:

\begin{equation}
    \text{argmax} : \R^k \to \mathcal{P}(C)
\end{equation}

Defined this way, we cannot necessarily consider $\argmax$ to be a function in general as the singleton outputs of argmax overlap in an undefined way with other sets from the power set. However, if we restrict our domain carefully, we can identify certain properties. 

Restricting to only the pre-image of the singletons, it should be clear that argmax is continuous. 

Indeed, restricted to the pre-image of any set in the power-set, argmax is continuous. 

Further, we can directly prove that the pre-image of an individual singleton is open. Observe that for any point whose image is a singleton, one element of the domain vector must exceed the others by $\varepsilon > 0$. We shall use the $\ell^1$ metric for distance, and thus if we restrict ourselves to a ball of radius $\varepsilon$, then all elements inside this ball will have that element still larger than the rest and thus map to the same singleton under argmax. Since the union of infinitely many open sets is open in $\R^k$, the union of all singleton pre-images is an open set. Conveniently this also provides proof that the union of all of the non-singleton sets in $\mathcal{P}(C)$ is a closed set. We will call this closed set the argmax Decision Boundary. 

Note : there are ways argmax can be forced to break ties, i.e. by ordering the 

Questions:

Is the decision boundary connected


\section{Defining Decision Boundaries}

\subsection{Complement Definition}

A point $x$ is in the \emph{decision interior} $D_f'$ for a classifier $f: \mathbb{R}^N -> \mathcal{C}$ if there exists $\delta > 0$ such that $\forall \epsilon < \delta$, $|f(B_\epsilon(x))| = 1$. 

The \emph{decision boundary} of a classifier $f$ is the closure of the complement of the decision interior $\overline{\{x : x \notin D_f'\}}$. 

\subsection{Constructive Definition}

A point $x$ is on the \emph{decision boundary} $D$ of a classifier $f$ if $\forall \epsilon > 0$, $|f(B_\epsilon(x))| \geq 2$.\\

A point $x$ is a \emph{binary decision point} if $\exists \delta > 0$ such that $\forall \epsilon > 0$ if $\epsilon < \delta$, then $|f(B_\epsilon(x))| = 2$. 

A point $x$ is on the \emph{$K$-decision boundary} $D^K$ of a classifier $f$ if $\exists \delta > 0$ such that $\forall \epsilon > 0$ if $\epsilon < \delta$, then $|f(B_\epsilon(x))| = K$. 

\subsection{Level Set Definition}

The decision boundary $D$ of a probability valued function $F$ is a union of all level sets $L_{c_1, c_2, a}$ defined by two classes $c_1$ and $c_2$ and a constant $a$ which satisfy two properties: First, given $x \in L_{c_1, c_2, a}$, $F(x)_{c_1} = F(x)_{c_2} = a$ where $a$ is a constant also defining the level set. Second, for all $c \notin \{c_1, c_2\}$, we have $a > F(x)_c$.   

\subsection{Images of Decision Boundaries}

We can consider a classification workflow $f$ from a data space $X$ (e.g. $\mathbb{R}^N$) using a model $F$ mapping the data space $X$ to a probability space $Y$ (e.g. $[0,1]^K$ where $K$ is the number of classes) and using argmax to convert continuous representations in $Y$ to discrete classes in the set of classes $\mathbb{C}$. 

\begin{align}
    X \myrightarrow{F} Y \myrightarrow{\text{argmax}} \mathcal{C}
\end{align}

In this way we define a usual discrete classifier $f = F \circ \text{argmax}$ 

The decision boundary $D$ is defined on $X$, however we may look at the image of the decision boundary under $F$. For example, if there are only two classes, then $Y = [0,1]^2$ and the decision boundary can be nicely visualized by the black line below: 

\begin{tikzpicture}
  \draw[->] (-0.5, 0) -- (3.5, 0) node[right] {$x$};
  \draw[->] (0, -0.5) -- (0, 3.5) node[above] {$y$};
  \node at (1, 2) (c1) {Class 1};
  \node at (2, 1) (c2) {Class 2};
  \draw[-, fill, blue, opacity=.3] (0, 3) -- (3, 3) -- (0, 0);
  \draw[-, fill, red, opacity=.3] (3, 0) -- (3, 3) -- (0, 0);
  \draw[scale=1, domain=0:3, smooth, variable=\x, black, line width=0.45mm] plot ({\x}, {\x});
  %\draw[scale=0.5, domain=-3:3, smooth, variable=\y, red]  plot ({\y*\y}, {\y});
\end{tikzpicture}

Furthermore, if the output of $F$ are \emph{probabilities} which add to one, then all points of $x$ will map to the orange line:

\begin{tikzpicture}
  \draw[->] (-0.5, 0) -- (3.5, 0) node[right] {$x$};
  \draw[->] (0, -0.5) -- (0, 3.5) node[above] {$y$};
  \node at (1, 2) (c1) {Class 1};
  \node at (2, 1) (c2) {Class 2};
  \draw[-, fill, blue, opacity=.3] (0, 3) -- (3, 3) -- (0, 0);
  \draw[-, fill, red, opacity=.3] (3, 0) -- (3, 3) -- (0, 0);
  \draw[scale=1, domain=0:3, smooth, variable=\x, black, line width=0.45mm] plot ({\x}, {\x});
  \draw[-, orange, line width=0.45mm] (0,3) -- (3, 0);
  %\draw[scale=0.5, domain=-3:3, smooth, variable=\y, red]  plot ({\y*\y}, {\y});
\end{tikzpicture}

We note that the point $(0.5, 0.5)$ is therefore the only point on the decision boundary for probability valued $F$. We may generalize to higher dimensions where all probability valued models $F$ will map into the the plane $x + y + z + \cdots = 1$ in $Y$ and the decision boundary will be partitioned into $K-1$ components, where the $K$-decision boundary is the intersection of this plane with the \emph{centroid} line $x = y = z = \cdots$ and the $2$-decision boundaries become planes intersecting at the same line. 

\section{Properties of Decision Boundaries}

In practice, decision boundaries have a variety of properties. The
decision boundary is a pre-image under an onto function that is not
1-1, which allows decision boundaries to vary in upto as many
dimensions as the data space. In practice, this will likely be many
fewer. In particular, decision boundaries should correspond with the
structure of the data. If the data is embedded within a k-manifold
within the input space, the decision boundary can be though of on the
dual space of that manifold.

The dual space of a $k$-manifold embedded in an $n$-dimensional Euclidean space is the space of differential $k$-forms on the manifold. More precisely, for a $k$-manifold $M$ embedded in an $n$-dimensional Euclidean space, the dual space is defined as the space of covariant $k$-tensors on $M$, denoted by $\Lambda^k(M)$, which consists of all linear maps from the tangent space of $M$ at each point to the real numbers.

In particular, when $M$ is a smooth $k$-dimensional manifold, $\Lambda^k(M)$ is the space of smooth $k$-forms on $M$, which can be locally expressed as linear combinations of differential forms of the form $dx_I = dx_{i_1} \wedge dx_{i_2} \wedge \cdots \wedge dx_{i_k}$, where the indices $i_1 < i_2 < \cdots < i_k$ denote the coordinates of a $k$-dimensional chart on $M$ and $dx_i$ denotes the differential of the $i$-th coordinate function.

Intuitively, a $k$-form on $M$ assigns to each $k$-dimensional oriented subspace of the tangent space at a point a signed volume, and the space of all such $k$-forms forms the dual space of $M$. This dual space is important in various areas of mathematics and physics, including differential geometry, topology, and gauge theory.

\subsection{Delaunay Decision Boundaries}

The simplest special case within this dual space is a classifier which
is defined using the Voronoi diagram for the dataset. We can use the
voronoi diagram to define a classifier for an arbitrary query point by
simply assigning it the class of the training point whose voronoi cell
contains it. This has several useful properties, though one in
particular stands out.

Given two points $x$ and $y$ in the training set $X$ which define a delaunay
triangulation and its corresponding voronoi diagram (which is the dual
of the delaunay triangulation) we can see that a line connecting $x$ to
$y$ must orthogonally cross the decision boundary -- which is exactly the voronoi
diagram of this dataset.

Proof:
\begin{proof}
Let $x$ and $y$ be two points in a dataset $X$ that share an edge in the Delaunay triangulation for $X$, and let $e$ be the edge they share in the Delaunay graph. Suppose that $e$ is not orthogonal to the face of the Voronoi diagram that $x$ and $y$ share. Then there exists a point $z$ in the interior of the Voronoi cell for $x$ and $y$ such that the line through $z$ and the midpoint of $e$ intersects the face of the Voronoi diagram at a point $p$.

Since $z$ is in the Voronoi cell for $x$ and $y$, it follows that $d(z, x) < d(z, y)$ (where $d$ is the Euclidean distance). But this contradicts the fact that $x$ and $y$ share an edge in the Delaunay triangulation, which implies that the circumcircle of the triangle formed by $x$, $y$, and $z$ does not contain any other points in $X$. In particular, this means that the circumcenter of this triangle lies on the perpendicular bisector of $e$, which implies that $e$ is orthogonal to the face of the Voronoi diagram that $x$ and $y$ share.

Therefore, we have shown that if $x$ and $y$ share an edge in the Delaunay triangulation for $X$, then the edge they share in the Delaunay graph must be orthogonal to the face of the Voronoi diagram that they share.
\end{proof}
It is immediately clear that for points not in the training set,
the line connecting them with eachother or with a point in the
training set need not cross orthogonal to the voronoi cell
boundaries. In order to talk clearly about such non-orthogonal
crossings, we will define
\begin{definition}
In arbitrary dimensional space, the \emph{angle of incidence} between a line and a plane is defined as the angle between the line and its projection onto the plane, measured in the plane.

More precisely, let $\mathbb{R}^n$ be an $n$-dimensional Euclidean space, let $\ell$ be a line in $\mathbb{R}^n$ with direction vector $\vec{v}$, and let $P$ be a plane in $\mathbb{R}^n$ with normal vector $\vec{n}$. Suppose that $\ell$ intersects $P$ at a point $Q$. Let $H$ be the orthogonal projection of $\ell$ onto $P$, and let $\theta$ be the angle between $\ell$ and $H$.

Then, the angle of incidence between $\ell$ and $P$ is defined as $\alpha = \frac{\pi}{2} - \theta$, where $\pi$ is the constant representing the ratio of the circumference of a circle to its diameter.

Note that when $n=3$, this definition reduces to the familiar definition of the angle of incidence between a line and a plane in three-dimensional space. However, the definition is valid for arbitrary dimensional space.
\end{definition}

and
\begin{definition}
The 
\end{definition}

\subsection{Level Set Definition}
\begin{definition}
The \emph{decision boundary} $D$ of a probability valued function $F$
is a union of all level sets $L_{c_1, c_2, a}$ defined by two classes
$c_1$ and $c_2$ and a constant $a$ which satisfy two properties:
First, given $x \in L_{c_1, c_2, a}$, $F(x)_{c_1} = F(x)_{c_2} = a$
where $a$ is a constant also defining the level set. Second, for all
$c \notin \{c_1, c_2\}$, we have $a > F(x)_c$. This is the
\emph{decision level set} for level $a$. For a given point $x$ on the
decision boundary of a function, the \emph{decision level} is the
value $a$ defining the level set of the decision boundary of which $x$
is a member.

\textbf{Note: } Any point $x$ can be in at most one level set of the
decision boundary. 

\end{definition}

\begin{definition}
  The \emph{dimension} of the decision boundary at a point $x$ is the
  number of dimensions needed to span $\{z : (x + z)$ is in the decision
    level $a$ of the level set containing $x\}$
\end{definition}

A primary property of interest in adversariall attacks is
``sharpness'' i.e. the property that a partition of a set which is
attributed to one class might stab needle-like into a partition of
another set. We will investigate this ``sharpness'' concept by
examining both the incident angle (the acuteness of angles in the
decision boundary) and the dimension of the decision boundary, since
both properties behave like one another. 

There is one conditional bound which is specifically for
voronoi cells which are not exterior to the voronoi diagram. Such
cells are bounded. The line connecting a point within a bounded cell
to the point defining any adjacent voronoi cell.

\subsection{Weighted Delaunay Decision Boundaries}
This simple voronoi classifier has the limitation that it only cares
about which individual training datapoint is closest to the query
point, but is not sensitive to the distribution of this data. If we
suppose that this data is distributed on a manifold with significant
co-dimension with respect to the ambient data space, then it would be
best to use a metric based on this manifold, so that distance among
the data, and hence the delaunay triangulation and the comensurate
voronoi cells would be determined by this metric and thus properly
sensitive to the underlying geometry of this distribution. Alas, this
is akin to having the generating function for nature. It cannot be
computed. So instead, we can take advantage of the Delaunay
triangulation with the usual euclidean metric as an approximation of
the lower dimensional manifold in this case.

This method is limited by the quality of the training dataset as a
sampling of the distribution in question. The Delaunay triangulation
is very sensitive to outliers from a distribution, meaning that our
samples must have relatively little noise in order to be treated as
appropriate samples from the low-dimensional manifold. Second,
Delaunay triangulations are unstable in high-dimensions where very
small triangles are more likely. Both of these problems are lessened
by using data which are sufficiently plentiful relative to the
dimension of the lower dimensional manifold and by requiring that they
do not have more than a small amount of noise to perturb them from the
low dimensional manifold. 

Suppose the lower dimensional manifold $M$ could be defined, and the
training dataset $X$ could be projected onto $M$. The decision
boundary partitioning $M$ would be a set of slices orthogonal to $M$
which would partition any training dataset $X$ into its appropriate
parts. In particular, for a sufficiently dense sampling $x$, we could
define this decision boundary by examining the data points immediately
on either side the decision boundary wherever they meet. We can define
an approximation of the decision boundary as the orthogonal partition
that we expect to be equidistant between adjacent points of different
classes for all samplings of training points. % todo refine this language
In fact, we can define this boundary in the limit using delaunay
triangulation:
\begin{definition}
  Let $M$ be a low dimensional manifold and let $X_{\varepsilon}$ be a
  sampling of points on $M$ for which the maximal edge length along
  its Delaunay triangulation $D_{\varepsilon}$ is
  $\varepsilon$. Given a query point $z$, the $\varepsilon-$Delaunay
  weight for class $i$, $w(z)_i$, is the sum of the barycentric coordinates of $z$
  relative to the vertices with label $i$ of the simplex of $D_{\varepsilon}$ which
  contains $z$. The weight vector $\varepsilon$ boundary level set for
  factor $a$, $B_{\varepsilon,a}$ is the level set $\{z \in M :$ for
  all $i$, we have $w(z)_i \leq a$ and for some $i,j$, $w(z)_i =
  w(z)_j = a\}$. The union of all such level sets over $a$ is the
  \emph{$\varepsilon-$Delaunay-Boundary} $B_{\varepsilon}$. 
  \end{definition}

  Remark, we can extend the decision boundary outside of $M$ by simply
  extending the Delaunay-Boundary using the usual euclidean metric. 

  \begin{theorem}
    Given a low dimensional manifold $M$, 
    \begin{align}
      \lim_{\varepsilon \to 0} B_{\varepsilon}(M) = B(M)
    \end{align}
    $B(M)$ is the decision boundary restricted to $M$. 
  \end{theorem}
  
In this way, a particular training set $X$ defines an approximation of
the general Delaunay Decision Boundary which is well defined outside
of $M$. If the decision boundary is smooth, then for a sufficiently
dense training set $X$ which is sufficiently close to $M$, this
approximation can be bounded by $\varepsilon$ and a lipshitz constant
coming from the mean value theorem on the decision boundary.

It is this approximate form of the decision boundary which we may in
practice evaluate. 

\subsection{Orthant and Wedge}

In order to study decision boundaries, we must talk about properties
related to how decision boundaries interact. We desire a test-object
whose dimensionality and acuteness of angle we can control. To this
end we will use the $k-$dimensional orthant:

\begin{definition}
  Given an integer $k$, the \emph{$k$-orthant} in $n$ dimensions is the set $\{x \in \mathbb{R}^{n}$
  such that for every natural number $i \leq k$, $x_i > 0\}$
  \end{definition}

This concept for an orthant can be extended to be acute in arbitrarily
many angles by tipping toward $x$ to form a wedge.

\begin{definition}
  Given integer $k$ and a set of $k-1$ angles $\Theta$, the \emph{$k-\Theta-$wedge} in $n$ dimensions is the set $\{x \in \mathbb{R}^{n}$
  such that $x_1 > 0$ and for every natural number $1 < i \leq k$,
  $x_i > x_1 \tan(\theta_{i-1})\}$. 
  \end{definition}

These objects allow us to control the dimensionality and acuteness of
a decision boundary to test decision boundary metrics. Another recipe
for analysis is standardizing the paths along which we will cross
decision boundaries. We will use two general paths relative to the
wedge for comparison: centerline and $x-$parallel:

\begin{definition}
  The \emph{centerline} $k-\Theta-$wedge crossing is defined along
  the line $x_1 = t$, for $1 < i \leq k$ $x_i = t
  \tan(\theta_{i-1}/2)$, and for $i > k$ $x_i = 0$.\\

  The \emph{$x-\varepsilon-$parallel} $k-\Theta-$wedge crossing is defined along
  the line $x_1 = t$, for $i > 1$ $x_i = \varepsilon$
\end{definition}

Although we can easily determine whether a point is inside or outside
the wedge simply by checking whether it satisfies the conditions
defining the wedge, we also wish to compute the projection or nearest
point on the wedge for an arbitrary query point. This involves solving
for the closest point to a convex object, which can be accomplished by
projection onto convex sets. 

Computing this projection requires we determine which inequalities
have been violated. Each inequality corresponds with a hyper-plane.
\begin{definition}
  Given a finite set of half-planes $Y_i$ in $\mathbb{R}^n$ and a point $x$,
  let $I$ contain all $i$ such that $x \notin Y_i$. Then since the
  intersection of any number of convex sets is convex, $Y_x = \cap_{i \in
    I} Y_i$ is a convex set. Furthermore, there is exactly one point
  $z$ with $|x - z| \leq |x - y|$ for every $y$ in $Y_x$. This is the
  \emph{projection} of $x$ onto $Y_x$.
\end{definition}

In order to compute this point in practice, we must first determine
all half-planes that do not contain $x$ and then perform orthogonal
projection in sequence along these half-planes using Projection onto
Convex Sets ~/cite{vonneuman-pocs}. 

\begin{lemma}
  If all half-planes $Y_i$ with corresponding normal vector $v_i$ have
  boundaries $B(Y_i)$ which are mutually orthogonal, i.e. if $\langle
  v_i, v_j\rangle = 0$ for every combination of $i$ and $j$, then
  the nearest point can be solved by iterative projection 
  \begin{align}
    \vectorproj[v_{i_1}]{(\vectorproj[v_{i_2}]{(\vectorproj[v_{i_3}]{...(x)})})}
  \end{align}
\end{lemma}
(~\cite{vonneuman-pocs})

In the case of the upper wedge, the boundaries are not mutually orthogonal, so
simple orthogonal projection is not sufficient. We must explore this
projection in more detail. Really, what we wish to do is project the
query point $x$ onto the intersection of all of its violated
boundaries. Iteratively, we can orthogonaly project onto the first
hyperplane. We will conduct our projection by subtracting a projection
onto a normal vector for each hyperplane. Given a point $x$, a
hyperplane $p_i$ and its normal vector $v_i$, we define 
\begin{align}
\vectorproj[p_i]{(x)} &= x - x \cdot v_i
\end{align}
The normal vectors for our wedge come in two forms. For the orthant,
all of the normals are of the form $v_i = e_i$. For the angled wedge planes,
they are all of the form $w_i = e_i \cos(\theta_i) - e_1
\sin(\theta_i)$ where $i > 1$. We immediately note that $v_i \cdot v_j
= 0$ for every natural number $i$ and $j$ less than the number of
planes $k$. However,
\begin{align}
  w_i \cdot w_j &= \langle e_i \cos(\theta_i) - e_1 \sin(\theta_i), e_j
                  \cos(\theta_j) - e_1 \sin(\theta_j)\rangle\\
                &= e_ie_j\cos(\theta_i)\cos(\theta_j) -
                  e_1e_j\cos(\theta_j)\sin(\theta_j) - e_1e_i
                  \cos(\theta_i)\sin(\theta_j) +
                  e_1^2\sin(\theta_j)\sin(\theta_i)\\
                &= e_1 \sin(\theta_j)\sin(\theta_i)\\
\end{align}
This means that none of the $w_j$ are orthogonal to each-other and
furthermore 
\begin{align}
  v_1 \cdot w_i &= \langle e_1, -e_1 \sin(\theta_i) + e_i
                  \cos(\theta_i) \rangle \\
                  &= -\sin(\theta_i)
\end{align}
We will leave this latter lack or orthogonality for last, and start by
determining how to sequentially orthogonally project onto the
$w_j$. Critically, we need only project onto the intersection of each
$w_i$ with all previously projected $w_j$. We begin by projecting
from within the plane defined by $w_i$ onto the plane defined by
$w_j$. These vectors are not orthogonal, so we must derive a new
plane and its normal vector $w_{ij}$ which is still orthogonal to $w_i$ but
shares the same intersection with the plane defined by $w_j$ along the
same edge. The conditions that must be satisfied are: 
\begin{align}
  w_{ij} \cdot w_j &= 0 \\
  w_{ij} \perp \cap(w_i, w_j)\\
  w_{ij} \cdot (e_1 + e_i \tan \theta_i + e_j \tan \theta_j) &= 0
\end{align}
This third condition is the requirement that $w_{ij}$ is orthogonal to all
vectors in the intersection of planes $i$ and $j$.

We'll attempt to solve these equations by using a variable $a$ to
account for the discrepency needed to solve these equations. 
\begin{align}
  w_{ij} &= w_j + a = e_j \cos \theta_j - e_1 \sin \theta_j + a\\
  a &= a_1e_1 + a_2e_2 + \cdots a_n e_n \\
  w_{ij} \cdot w_i &= \sin \theta_j\sin\theta_i - a_1 \sin\theta_j +
                     a_i \cos \theta_i = 0\\
  w_{ij} \cdot (e_1 + e_i \tan \theta_i + e_j \tan \theta_j) &= a_1 -
                                                               a_i
                                                               \tan
                                                               \theta_i
                                                               + a_j
                                                               \tan \theta_j
\end{align}
Letting $a_1 \neq 0$ requires that $a = e_1 \sin \theta_j - e_j \cos
\theta_j$ which is a degenerate case, so let $a_1 = 0$. For every
$a_k$ not involved in the intersection of planes, they will have zero
dot product, so we can let them all be 0. Then
\begin{align}
  -a_i \cos \theta_i &= \sin \theta_j \sin \theta_i\\
  a_i &= -\sin \theta_j \tan \theta_i\\
  a_j \tan \theta_j &= \sin \theta_j \tan^2 \theta_i\\
  a_j &= \cos \theta_j \tan^2 \theta_i\\
  w_{ij} &= w_j - e_i \sin \theta_j \tan \theta_i + e_j \cos \theta_j
           \tan^2 \theta_i
\end{align}
Projecting once more onto $w_{k}$ which also shares an intersection
with $w_i$ and $w_j$, we gain one parameter and one degree of
freedom.
\begin{align}
  w_{ijk} &= w_k + a = e_k \cos \theta_k - e_1 \sin \theta_k + a\\
  a &= a_1e_1 + a_2e_2 + \cdots a_n e_n \\
  w_{ijk} \cdot w_i &= \sin \theta_k\sin\theta_i - a_1 \sin\theta_k +
                     a_i \cos \theta_i = 0\\
  w_{ijk} \cdot w_j &= \sin \theta_k\sin\theta_j - a_1 \sin\theta_j +
                     a_j \cos \theta_j = 0\\
  w_{ijk} \cdot (e_1 + e_i \tan \theta_i + e_j \tan \theta_j) &= a_1 +
                                                               a_i
                                                               \tan
                                                               \theta_i
                                                               + a_j
                                                               \tan
                                                                \theta_j
                                                                + a_k
                                                                \tan \theta_k
\end{align}
Now, again letting $a_1 = 0$ to avoid a degenerate case and letting
all other components of $a$ be zero, we have:
\begin{align}
  -a_i \cos \theta_i &= \sin \theta_k \sin \theta_i\\
  a_i &= -\sin \theta_k \tan \theta_i\\
  -a_j \cos \theta_j &= \sin \theta_k \sin \theta_j\\
  a_j &= -\sin \theta_k \tan \theta_j\\
  a_k \tan \theta_k &= \sin \theta_k \tan^2 \theta_i + \sin \theta_k \tan^2 \theta_j\\
  a_k &= \cos \theta_k (\tan^2 \theta_i + \tan^2 \theta_j)\\
  w_{ij} = w_j &- e_i \sin \theta_k \tan \theta_i\\
              &- e_j \sin \theta_k \tan \theta_j\\
              &+ e_k \cos \theta_k (\tan^2 \theta_i + \tan^2 \theta_j)
\end{align}
We see now that we can project an arbitrary sequence of such
intersecting surfaces with each $w_{i...k}$ with $a_i = -\sin \theta_k
\tan \theta_i$ for $i$ less than $k$ and $a_k = \cos \theta_k (\sum_{i
  = 1}^k\tan^2 \theta_i)$. 
Now for our projection algorithm, we first determine if all planes are
satisfied ($x \cdot v_i \geq 0$ and $x \cdot w_i \leq 0$ for every
$i$.) If they are, then we will project onto each plane and pick the
nearest point. If they are not all satisfied, now we'll check each
pair of planes $w_i$ and $v_i$. If both are satisfied, we will skip
them, if both are violated, we will set the coordinate in their native
direction $e_i$ to 0. When only one of the two planes for all compute all planes that are
violated by the position of each query point. For each pair of related
planes $w_i$ and $v_i$, there are three cases. Both satisfied, Both
violated, or either or. In the case that both are violated, i.e. $x
\cdot v_i < 0$, then $x_1 < 0$, which is to say the nearest point
within the wedge in these coordinates will be on the origin. When both
conditions are satisfied, we will ignore this plane except 


%%%%%%%%%%%%%%%%

Now, performing orthogonal projection,
we can orthogonally project in sequence for all half-planes not
containing $x$ except for $v_1$ since $e_1$ is not orthogonal to any
of the wedge planes. Once we have projected onto all other violated
planes, if the projection onto $e_1$ is negative, this will mean that
the nearest point to $x$ is the origin. For $i \neq 1$, all these
projections are of the first form. $x - \sum_{i} x \cdot e_i$. The
first projection of the second form can be done by simple orthogonal
projection, however in order to perform the next projection, we must
project onto the intersection of the two half-planes without leaving
the first plane. We'll need a new plane which is orthogonal to the
first plane, but has the same intersection with the second plane. We
can compute what is missing to make this projection orthogonal. We
have
\begin{align}
  w_i \cdot w_j &= \langle e_i \sin(\theta_i) - e_1 \cos(\theta_i), e_j
                  \sin(\theta_j) - e_1 \cos(\theta_j)\rangle\\
                &= e_ie_j\sin(\theta_i)\sin(\theta_j) -
                  e_1e_j\sin(\theta_j)\cos(\theta_j) - e_1e_i
                  \sin(\theta_i)\cos(\theta_j) +
                  e_1^2\cos(\theta_j)\cos(\theta_i)\\
                &= e_1 \cos(\theta_j)\cos(\theta_i)\\
\end{align}

We can solve for a perturbation in the $e_1$ direction which will make
these two normal vectors orthogonal but due to preserving 

% \section{exploring boundary curvature with Random Walks}

% To analyze decision boundary curvature, we will project samples of points onto the decision boundary and then use Singular Value Decomposition to analyze the \emph{projected points}. In general, this process will involve first selecting two images $x_1$ and $x_2$ for which $C(x_1) \neq C(x_2)$. A point $x_b$ for which $C(x_b)$ is ambiguous between $C(x_1)$ and $C(x_2)$. The resulting sample $X$ will be projected to the decision boundary by either computing a loss function that is minimized when each of the classes $C(X)$ flip from $C(x_1)$ to $C(x_2)$ or vice versa respectively and performing gradient descent, or by interpolating to the parent point of opposite class (so for $x \in X$, if $C(x) = C(x_1)$, we will interpolate from $x$ to $x_2$). 

% Once a projection has been found, we will take the singular value decomposition (SVD) of this sample and examine it for degeneracy. 


% Initial comparison of SVDs of decision boundary points yields a single dominant singular value which corresponds with the content of the original image on the boundary. All random noise appears to be mostly orthogonal to this. 

% Once this vector is removed, the remaining signal is simply the adversarial attack information. 

% To get a set of singular vectors which to not emphasize the image content, we take random differences among the sampled images and take the SVD of those random differences. 

% In these first 10 images, this procedure is carried out on the orthant, where samples are generated with mean 0 and are projected onto orthants with increasing numbers of dimensions. We can see a very clear dropped set of singular values smaller than the rest, which indicate the number of degenerate dimensions. In each of these cases, the dropped singular values match the dimension of the orthant. 

% Experiment : A valid experiment here is to measure the difference between the images and the projection to get -- in this case -- normal vectors to the orthant for each image sampled. The SVD of these normals can be computed to determine the number of dimensions in the projecetion operation. This same procedure can be caried out later in the real practical image projections, although in that case orthogonality is not guaranteed. 

% \includegraphics[width=8cm]{c4_figures/e03-SVD-Orthant_origin-dim-cropped1.png}
% \includegraphics[width=9cm]{c4_figures/e03-SVD-Orthant_origin-dim-cropped2.png}
% \includegraphics[width=9cm]{c4_figures/e03-SVD-Orthant_origin-dim-cropped3.png}
% \includegraphics[width=9cm]{c4_figures/e03-SVD-Orthant_origin-dim-cropped4.png}
% \includegraphics[width=9cm]{c4_figures/e03-SVD-Orthant_origin-dim-cropped5.png}
% \includegraphics[width=9cm]{c4_figures/e03-SVD-Orthant_origin-dim-cropped6.png}
% \includegraphics[width=9cm]{c4_figures/e03-SVD-Orthant_origin-dim-cropped7.png}
% \includegraphics[width=9cm]{c4_figures/e03-SVD-Orthant_origin-dim-cropped8.png}
% \includegraphics[width=9cm]{c4_figures/e03-SVD-Orthant_origin-dim-cropped9.png}
% \includegraphics[width=9cm]{c4_figures/e03-SVD-Orthant_origin-dim-cropped10.png}

% There is a question of how best to measure "normal" vectors for each projection. The most direct computation is to take a sample with small variance around each point on the decision boundary and solve least squares of each of these samples. We have previously observed that \emph{most} of the decision boundary is locally planar. 

% It remains to compare these computed normals with other known quantities, e.g. the gradient computed with respect to adversarial loss functions and the difference between each sampled image and its resultant projection. In addition, it remains to compare the normals of multiple nearby images to determine at what radius of sample the decision boundary begins to show curvature.\\

% The following image shows singular values in order for a sample around a decision boundary image in MNIST generated by interpolating from a test image to an adversarial image generated from it. This plot is dominated by the natural distribution of singular values for a gaussian and also by the original image information which can be seen as a huge singular value on the far left. We will address both of these factors in following plots. \\

% \includegraphics[width=14cm]{c4_figures/SVD-rand_diff-decision_boundary_uvar-1.0-index-0-image-999.png}

% The following plots are generated with a new distribution to replace the gaussian. This "Flat SVD" distribution is generated by first taking a gaussian sample representable by a matrix $X$, then taking the SVD of this gaussian sample $U \Sigma V = X$, replacing $\Sigma$ by $|\Sigma|_2 I$. This distribution has the property that its SVD is flat, while maintaining the Frobenius norm of $X$. This helps to highlight degeneracy in singular values. \\

% These first two plots are generated by sampling around a decision boundary image found by interpolating between two test images (rather than a test image and an adversarial example generated from it). We note that the SVD contains two degernate values. These seem to correpond with the two original images of the interpolation. 

% \includegraphics[width=14cm]{c4_figures/e05-SVD-uniform-rand_diff-decision_boundary_uvar-0.001-index-0-image-999.png}

% \includegraphics[width=14cm]{c4_figures/e05-SVD-uniform-rand_diff-decision_boundary_uvar-0.001-index-0-image-999-cropped.png}


% These last two images are generated with the flattened distribution 

% \includegraphics[width=14cm]{c4_figures/e06-SVD-uniform-rand_diff-decision_boundary_uvar-0.0001-index-0-image-999-cropped.png}

% \includegraphics[width=14cm]{c4_figures/e06-SVD-uniform-rand_diff-decision_boundary_uvar-0.0001-index-0-image-999.png}

% What these experiments tell us is that most of the time when we cross a decision oundary in the MNIST Dataset, we are crossing at a plane, however if we examine a slightly larger ball around a given point, it will intersect the decision boundary at many other places. 

% \section{Re-Examining Persistence}

% A movivating picture in this research is an image generated while interpolating persistence in the beginning of this research. 

% \includegraphics[width=15cm]{c4_figures/persistence_interpolation-IMNET-class-11-vgg16-BIM-48-attack_data-001 (2).png}

% The next objective is to examine this particular case with our random walk and projection Tools. 

% We also wish to augment these tools to include 

% %%%%%%%%%%%%%%%%%

% \subsection{in probability space}
% \subsection{in image space}
% \section{define orthants}
% \section{skewness}

% \section{sampling decision boundaries and analyzing dimensionality
% with PCA}

% \section{neural network attack gradients versus decision boundaries}

% \section{skewed orthant recreates persistence picture (?). }
% \section{measuring skewness of ANNs}
% \section{Relate skewness with dimpled manifold and features not bugs papers}


% turn observations into are they a definition, a theorem, or a discussion

% decision\_boundary crossing


==> Chapters/ChapterInstructions.tex <==
% Chapter 1

\chapter{Type the title for Chapter 1 here} % Main chapter title

\label{Chapter1} % For referencing the chapter elsewhere, use \ref{Chapter1} 

%----------------------------------------------------------------------------------------

% Define some commands to keep the formatting separated from the content 
\newcommand{\keyword}[1]{\textbf{#1}}
\newcommand{\tabhead}[1]{\textbf{#1}}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\file}[1]{\texttt{\bfseries#1}}
\newcommand{\option}[1]{\texttt{\itshape#1}}

%----------------------------------------------------------------------------------------

\section{Welcome and Thank You}
Welcome to this \LaTeX{} Thesis Template, a beautiful and easy to use template for writing a thesis using the \LaTeX{} typesetting system.

If you are writing a thesis (or will be in the future) and its subject is technical or mathematical (though it doesn't have to be), then creating it in \LaTeX{} is highly recommended as a way to make sure you can just get down to the essential writing without having to worry over formatting or wasting time arguing with your word processor.

\LaTeX{} is easily able to professionally typeset documents that run to hundreds or thousands of pages long. With simple mark-up commands, it automatically sets out the table of contents, margins, page headers and footers and keeps the formatting consistent and beautiful. One of its main strengths is the way it can easily typeset mathematics, even \emph{heavy} mathematics. Even if those equations are the most horribly twisted and most difficult mathematical problems that can only be solved on a super-computer, you can at least count on \LaTeX{} to make them look stunning.

%----------------------------------------------------------------------------------------

\section{Learning \LaTeX{}}

\LaTeX{} is not a \textsc{wysiwyg} (What You See is What You Get) program, unlike word processors such as Microsoft Word or Apple's Pages. Instead, a document written for \LaTeX{} is actually a simple, plain text file that contains \emph{no formatting}. You tell \LaTeX{} how you want the formatting in the finished document by writing in simple commands amongst the text, for example, if I want to use \emph{italic text for emphasis}, I write the \verb|\emph{text}| command and put the text I want in italics in between the curly braces. This means that \LaTeX{} is a \enquote{mark-up} language, very much like HTML.

\subsection{A (not so short) Introduction to \LaTeX{}}

If you are new to \LaTeX{}, there is a very good eBook -- freely available online as a PDF file -- called, \enquote{The Not So Short Introduction to \LaTeX{}}. The book's title is typically shortened to just \emph{lshort}. You can download the latest version (as it is occasionally updated) from here:
\url{http://www.ctan.org/tex-archive/info/lshort/english/lshort.pdf}

It is also available in several other languages. Find yours from the list on this page: \url{http://www.ctan.org/tex-archive/info/lshort/}

It is recommended to take a little time out to learn how to use \LaTeX{} by creating several, small `test' documents, or having a close look at several templates on:\\ 
\url{http://www.LaTeXTemplates.com}\\ 
Making the effort now means you're not stuck learning the system when what you \emph{really} need to be doing is writing your thesis.

\subsection{A Short Math Guide for \LaTeX{}}

If you are writing a technical or mathematical thesis, then you may want to read the document by the AMS (American Mathematical Society) called, \enquote{A Short Math Guide for \LaTeX{}}. It can be found online here:
\url{http://www.ams.org/tex/amslatex.html}
under the \enquote{Additional Documentation} section towards the bottom of the page.

\subsection{Common \LaTeX{} Math Symbols}
There are a multitude of mathematical symbols available for \LaTeX{} and it would take a great effort to learn the commands for them all. The most common ones you are likely to use are shown on this page:
\url{http://www.sunilpatel.co.uk/latex-type/latex-math-symbols/}

You can use this page as a reference or crib sheet, the symbols are rendered as large, high quality images so you can quickly find the \LaTeX{} command for the symbol you need.

\subsection{\LaTeX{} on a Mac}
 
The \LaTeX{} distribution is available for many systems including Windows, Linux and Mac OS X. The package for OS X is called MacTeX and it contains all the applications you need -- bundled together and pre-customized -- for a fully working \LaTeX{} environment and work flow.
 
MacTeX includes a custom dedicated \LaTeX{} editor called TeXShop for writing your `\file{.tex}' files and BibDesk: a program to manage your references and create your bibliography section just as easily as managing songs and creating playlists in iTunes.

%----------------------------------------------------------------------------------------

\section{Getting Started with this Template}

If you are familiar with \LaTeX{}, then you should explore the directory structure of the template and then proceed to place your own information into the \emph{THESIS INFORMATION} block of the \file{Dissertation.tex} file. You can then modify the rest of this file to your unique specifications based on your degree/university. Section \ref{FillingFile} on page \pageref{FillingFile} will help you do this. Make sure you also read section \ref{ThesisConventions} about thesis conventions to get the most out of this template.

If you are new to \LaTeX{} it is recommended that you carry on reading through the rest of the information in this document.

Before you begin using this template you should ensure that its style complies with the thesis style guidelines imposed by your institution. In most cases this template style and layout will be suitable. If it is not, it may only require a small change to bring the template in line with your institution's recommendations. These modifications will need to be done on the \file{DoctoralThesis.cls} file.

\subsection{About this Template}

This \LaTeX{} Thesis Template is originally based and created around a \LaTeX{} style file created by Steve R.\ Gunn from the University of Southampton (UK), department of Electronics and Computer Science. You can find his original thesis style file at his site, here:
\url{http://www.ecs.soton.ac.uk/~srg/softwaretools/document/templates/}

Steve's \file{ecsthesis.cls} was then taken by Sunil Patel who modified it by creating a skeleton framework and folder structure to place the thesis files in. The resulting template can be found on Sunil's site here:
\url{http://www.sunilpatel.co.uk/thesis-template}

Sunil's template was made available through \url{http://www.LaTeXTemplates.com} where it was modified many times based on user requests and questions. Version 2.0 and onwards of this template represents a major modification to Sunil's template and is, in fact, hardly recognizable. The work to make version 2.0 possible was carried out by \href{mailto:vel@latextemplates.com}{Vel} and Johannes Böttcher.

\emph{NOTE: This template was modified from its original version to comply with the standards of the University of Arizona Graduate College in January, 2019. Please check for updated standards and make necessary changes before embarking on your own dissertation writing.}
%----------------------------------------------------------------------------------------

\section{What this Template Includes}

\subsection{Folders}

This template comes as a single zip file that expands out to several files and folders. The folder names are mostly self-explanatory:

\keyword{Appendices} -- this is the folder where you put the appendices. Each appendix should go into its own separate \file{.tex} file. An example and template are included in the directory.

\keyword{Chapters} -- this is the folder where you put the thesis chapters. A thesis usually has about six chapters, though there is no hard rule on this. Each chapter should go in its own separate \file{.tex} file and they can be split as:
\begin{itemize}
\item Chapter 1: Introduction to the thesis topic
\item Chapter 2: Background information and theory
\item Chapter 3: (Laboratory) experimental setup
\item Chapter 4: Details of experiment 1
\item Chapter 5: Details of experiment 2
\item Chapter 6: Discussion of the experimental results
\item Chapter 7: Conclusion and future directions
\end{itemize}
This chapter layout is specialized for the experimental sciences, your discipline may be different.

\keyword{Figures} -- this folder contains all figures for the thesis. These are the final images that will go into the thesis document.

\subsection{Files}

Included are also several files, most of them are plain text and you can see their contents in a text editor. After initial compilation, you will see that more auxiliary files are created by \LaTeX{} or BibTeX and which you don't need to delete or worry about:

\keyword{example.bib} -- this is an important file that contains all the bibliographic information and references that you will be citing in the thesis for use with BibTeX. You can write it manually, but there are reference manager programs available that will create and manage it for you. Bibliographies in \LaTeX{} are a large subject and you may need to read about BibTeX before starting with this. Many modern reference managers will allow you to export your references in BibTeX format which greatly eases the amount of work you have to do.

\keyword{DoctoralThesis.cls} -- this is an important file. It is the class file that tells \LaTeX{} how to format the thesis. 

\keyword{Dissertation.pdf} -- this is your beautifully typeset thesis (in the PDF file format) created by \LaTeX{}. It is supplied in the PDF with the template and after you compile the template you should get an identical version.

\keyword{Dissertation.tex} -- this is an important file. This is the file that you tell \LaTeX{} to compile to produce your thesis as a PDF file. It contains the framework and constructs that tell \LaTeX{} how to layout the thesis. It is heavily commented so you can read exactly what each line of code does and why it is there. After you put your own information into the \emph{THESIS INFORMATION} block -- you have now started your thesis!

Files that are \emph{not} included, but are created by \LaTeX{} as auxiliary files include:

\keyword{Dissertation.aux} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file.

\keyword{Dissertation.bbl} -- this is an auxiliary file generated by BibTeX, if it is deleted, BibTeX simply regenerates it when you run the \file{Dissertation.aux} file. Whereas the \file{.bib} file contains all the references you have, this \file{.bbl} file contains the references you have actually cited in the thesis and is used to build the bibliography section of the thesis.

\keyword{Dissertation.blg} -- this is an auxiliary file generated by BibTeX, if it is deleted BibTeX simply regenerates it when you run the main \file{.aux} file.

\keyword{Dissertation.lof} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file. It tells \LaTeX{} how to build the \emph{List of Figures} section.

\keyword{Dissertation.log} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file. It contains messages from \LaTeX{}, if you receive errors and warnings from \LaTeX{}, they will be in this \file{.log} file.

\keyword{Dissertation.lot} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file. It tells \LaTeX{} how to build the \emph{List of Tables} section.

\keyword{Dissertation.out} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file.

So from this long list, only the files with the \file{.bib}, \file{.cls} and \file{.tex} extensions are the most important ones. The other auxiliary files can be ignored or deleted as \LaTeX{} and BibTeX will regenerate them.

%----------------------------------------------------------------------------------------

\section{Filling in Your Information in the \file{Dissertation.tex} File}\label{FillingFile}

You will need to personalize the thesis template and make it your own by filling in your own information. This is done by editing the \file{Dissertation.tex} file in a text editor or your favorite LaTeX environment.

Open the file and scroll down to the third large block titled \emph{THESIS INFORMATION} where you can see the entries for \emph{University Name}, \emph{Department Name}, etc \ldots

Fill out the information about yourself, your group and institution. You can also insert web links, if you do, make sure you use the full URL, including the \code{http://} for this. If you don't want these to be linked, simply remove the \verb|\href{url}{name}| and only leave the name.

When you have done this, save the file and recompile \code{Dissertation.tex}. All the information you filled in should now be in the PDF, complete with web links. You can now begin your thesis proper!

%----------------------------------------------------------------------------------------

\section{The \code{Dissertation.tex} File Explained}

The \file{Dissertation.tex} file contains the structure of the thesis. There are plenty of written comments that explain what pages, sections and formatting the \LaTeX{} code is creating. Each major document element is divided into commented blocks with titles in all capitals to make it obvious what the following bit of code is doing. Initially there seems to be a lot of \LaTeX{} code, but this is all formatting, and it has all been taken care of so you don't have to do it.

Begin by checking that your information on the title page is correct. For the thesis declaration, your institution may insist on something different than the text given. If this is the case, just replace what you see with what is required in the \emph{DECLARATION PAGE} block.

Then comes a page which contains a funny quote. You can put your own, or quote your favorite scientist, author, person, and so on. Make sure to put the name of the person who you took the quote from.

Following this is the abstract page which summarizes your work in a condensed way and can almost be used as a standalone document to describe what you have done. The text you write will cause the heading to move up so don't worry about running out of space.

Next come the acknowledgements. On this page, write about all the people who you wish to thank (not forgetting parents, partners and your advisor/supervisor).

The contents pages, list of figures and tables are all taken care of for you and do not need to be manually created or edited. The next set of pages are more likely to be optional and can be deleted since they are for a more technical thesis: insert a list of abbreviations you have used in the thesis, then a list of the physical constants and numbers you refer to and finally, a list of mathematical symbols used in any formulae. Making the effort to fill these tables means the reader has a one-stop place to refer to instead of searching the internet and references to try and find out what you meant by certain abbreviations or symbols.

The list of symbols is split into the Roman and Greek alphabets. Whereas the abbreviations and symbols ought to be listed in alphabetical order (and this is \emph{not} done automatically for you) the list of physical constants should be grouped into similar themes.

The next page contains a one line dedication. Who will you dedicate your thesis to?

Finally, there is the block where the chapters are included. Uncomment the lines (delete the \code{\%} character) as you write the chapters. Each chapter should be written in its own file and put into the \emph{Chapters} folder and named \file{Chapter1}, \file{Chapter2}, etc\ldots Similarly for the appendices, uncomment the lines as you need them. Each appendix should go into its own file and placed in the \emph{Appendices} folder.

After the preamble, chapters and appendices finally comes the bibliography. The bibliography style (called \option{authoryear}) is used for the bibliography and is a fully featured style that will even include links to where the referenced paper can be found online. Do not underestimate how grateful your reader will be to find that a reference to a paper is just a click away. Of course, this relies on you putting the URL information into the BibTeX file in the first place.

%----------------------------------------------------------------------------------------

\section{Thesis Features and Conventions}\label{ThesisConventions}

To get the best out of this template, there are a few conventions that you may want to follow.

One of the most important (and most difficult) things to keep track of in such a long document as a thesis is consistency. Using certain conventions and ways of doing things (such as using a Todo list) makes the job easier. Of course, all of these are optional and you can adopt your own method.

\subsection{Printing Format}

This thesis template is designed for double sided printing (i.e. content on the front and back of pages) as most theses are printed and bound this way. Switching to one sided printing is as simple as uncommenting the \option{oneside} option of the \code{documentclass} command at the top of the \file{Dissertation.tex} file. You may then wish to adjust the margins to suit specifications from your institution.

The headers for the pages contain the page number on the outer side (so it is easy to flick through to the page you want) and the chapter name on the inner side.

The text is set to 12 point by default with double line spacing, again, you can tune the text size and spacing should you want or need to using the options at the very start of \file{Dissertation.tex}. The spacing can be changed similarly by replacing the \option{singlespacing} with \option{onehalfspacing} or \option{doublespacing}.

\subsection{Using US Letter Paper}

The paper size used in the template is letter, which is the standard size in United States. If you are using this thesis template elsewhere and particularly in Europe, then you may have to change the US Letter paper size to the A4 size. This can be done in the margins settings section in \file{Dissertation.tex}.

Due to the differences in the paper size, the resulting margins may be different to what you like or require (as it is common for institutions to dictate certain margin sizes). If this is the case, then the margin sizes can be tweaked by modifying the values in the same block as where you set the paper size. Now your document should be set up for US Letter paper size with suitable margins.

\subsection{References}

The \code{biblatex} package is used to format the bibliography and inserts references such as this one \parencite{Reference1}. The options used in the \file{Dissertation.tex} file mean that the in-text citations of references are formatted with the author(s) listed with the date of the publication. Multiple references are separated by semicolons (e.g. \parencite{Reference2, Reference1}) and references with more than three authors only show the first author with \emph{et al.} indicating there are more authors (e.g. \parencite{Reference3}). This is done automatically for you. To see how you use references, have a look at the \file{Chapter1.tex} source file. Many reference managers allow you to simply drag the reference into the document as you type.

Scientific references should come \emph{before} the punctuation mark if there is one (such as a comma or period). The same goes for footnotes\footnote{Such as this footnote, here down at the bottom of the page.}. You can change this but the most important thing is to keep the convention consistent throughout the thesis. Footnotes themselves should be full, descriptive sentences (beginning with a capital letter and ending with a full stop). The APA6 states: \enquote{Footnote numbers should be superscripted, [...], following any punctuation mark except a dash.} The Chicago manual of style states: \enquote{A note number should be placed at the end of a sentence or clause. The number follows any punctuation mark except the dash, which it precedes. It follows a closing parenthesis.}

The bibliography is typeset with references listed in alphabetical order by the first author's last name. This is similar to the APA referencing style. To see how \LaTeX{} typesets the bibliography, have a look at the very end of this document (or just click on the reference number links in in-text citations).

\subsubsection{A Note on bibtex}

The bibtex backend used in the template by default does not correctly handle unicode character encoding (i.e. "international" characters). You may see a warning about this in the compilation log and, if your references contain unicode characters, they may not show up correctly or at all. The solution to this is to use the biber backend instead of the outdated bibtex backend. This is done by finding this in \file{Dissertation.tex}: \option{backend=bibtex} and changing it to \option{backend=biber}. You will then need to delete all auxiliary BibTeX files and navigate to the template directory in your terminal (command prompt). Once there, simply type \code{biber main} and biber will compile your bibliography. You can then compile \file{Dissertation.tex} as normal and your bibliography will be updated. An alternative is to set up your LaTeX editor to compile with biber instead of bibtex, see \href{http://tex.stackexchange.com/questions/154751/biblatex-with-biber-configuring-my-editor-to-avoid-undefined-citations/}{here} for how to do this for various editors.

\subsection{Tables}

Tables are an important way of displaying your results, below is an example table which was generated with this code:

{\small
\begin{verbatim}
\begin{table}
\caption{The effects of treatments X and Y on the four groups studied.}
\label{tab:treatments}
\centering
\begin{tabular}{l l l}
\toprule
\tabhead{Groups} & \tabhead{Treatment X} & \tabhead{Treatment Y} \\
\midrule
1 & 0.2 & 0.8\\
2 & 0.17 & 0.7\\
3 & 0.24 & 0.75\\
4 & 0.68 & 0.3\\
\bottomrule\\
\end{tabular}
\end{table}
\end{verbatim}
}

\begin{table}
\caption{The effects of treatments X and Y on the four groups studied.}
\label{tab:treatments}
\centering
\begin{tabular}{l l l}
\toprule
\tabhead{Groups} & \tabhead{Treatment X} & \tabhead{Treatment Y} \\
\midrule
1 & 0.2 & 0.8\\
2 & 0.17 & 0.7\\
3 & 0.24 & 0.75\\
4 & 0.68 & 0.3\\
\bottomrule\\
\end{tabular}
\end{table}

You can reference tables with \verb|\ref{<label>}| where the label is defined within the table environment. See \file{Chapter1.tex} for an example of the label and citation (e.g. Table~\ref{tab:treatments}).

\subsection{Figures}

There will hopefully be many figures in your thesis (that should be placed in the \emph{Figures} folder). The way to insert figures into your thesis is to use a code template like this:
\begin{verbatim}
\begin{figure}
\centering
\includegraphics{Figures/Electron}
\decoRule
\caption[An Electron]{An electron (artist's impression).}
\label{fig:Electron}
\end{figure}
\end{verbatim}
Also look in the source file. Putting this code into the source file produces the picture of the electron that you can see in the figure below.

\begin{figure}[th]
\centering
\includegraphics{Figures/Electron}
\decoRule
\caption[An Electron]{An electron (artist's impression).}
\label{fig:Electron}
\end{figure}

Sometimes figures don't always appear where you write them in the source. The placement depends on how much space there is on the page for the figure. Sometimes there is not enough room to fit a figure directly where it should go (in relation to the text) and so \LaTeX{} puts it at the top of the next page. Positioning figures is the job of \LaTeX{} and so you should only worry about making them look good!

Figures usually should have captions just in case you need to refer to them (such as in Figure~\ref{fig:Electron}). The \verb|\caption| command contains two parts, the first part, inside the square brackets is the title that will appear in the \emph{List of Figures}, and so should be short. The second part in the curly brackets should contain the longer and more descriptive caption text.

The \verb|\decoRule| command is optional and simply puts an aesthetic horizontal line below the image. If you do this for one image, do it for all of them.

\LaTeX{} is capable of using images in pdf, jpg and png format.

\subsection{Typesetting mathematics}

If your thesis is going to contain heavy mathematical content, be sure that \LaTeX{} will make it look beautiful, even though it won't be able to solve the equations for you.

The \enquote{Not So Short Introduction to \LaTeX} (available on \href{http://www.ctan.org/tex-archive/info/lshort/english/lshort.pdf}{CTAN}) should tell you everything you need to know for most cases of typesetting mathematics. If you need more information, a much more thorough mathematical guide is available from the AMS called, \enquote{A Short Math Guide to \LaTeX} and can be downloaded from:
\url{ftp://ftp.ams.org/pub/tex/doc/amsmath/short-math-guide.pdf}

There are many different \LaTeX{} symbols to remember, luckily you can find the most common symbols in \href{http://ctan.org/pkg/comprehensive}{The Comprehensive \LaTeX~Symbol List}.

You can write an equation, which is automatically given an equation number by \LaTeX{} like this:
\begin{verbatim}
\begin{equation}
E = mc^{2}
\label{eqn:Einstein}
\end{equation}
\end{verbatim}

This will produce Einstein's famous energy-matter equivalence equation:
\begin{equation}
E = mc^{2}
\label{eqn:Einstein}
\end{equation}

All equations you write (which are not in the middle of paragraph text) are automatically given equation numbers by \LaTeX{}. If you don't want a particular equation numbered, use the unnumbered form:
\begin{verbatim}
\[ a^{2}=4 \]
\end{verbatim}

%----------------------------------------------------------------------------------------

\section{Sectioning and Subsectioning}

You should break your thesis up into nice, bite-sized sections and subsections. \LaTeX{} automatically builds a table of Contents by looking at all the \verb|\chapter{}|, \verb|\section{}|  and \verb|\subsection{}| commands you write in the source.

The Table of Contents should only list the sections to three (3) levels. A \verb|chapter{}| is level zero (0). A \verb|\section{}| is level one (1) and so a \verb|\subsection{}| is level two (2). In your thesis it is likely that you will even use a \verb|subsubsection{}|, which is level three (3). The depth to which the Table of Contents is formatted is set within \file{DoctoralThesis.cls}. If you need this changed, you can do it in \file{Dissertation.tex}.

%----------------------------------------------------------------------------------------

\section{In Closing}

You have reached the end of this mini-guide. You can now rename or overwrite this pdf file and begin writing your own \file{Chapter1.tex} and the rest of your thesis. The easy work of setting up the structure and framework has been taken care of for you. It's now your job to fill it out!

Good luck and have lots of fun!

\begin{flushright}
Guide written by ---\\
Sunil Patel: \href{http://www.sunilpatel.co.uk}{www.sunilpatel.co.uk}\\
Vel: \href{http://www.LaTeXTemplates.com}{LaTeXTemplates.com}
\end{flushright}


==> Chapters/ch3leftover.tex <==
\section{Stability and Persistence} \label{sec:stab}
In this section we define a notion of stability of classification of a point under a given classification model. In the following, $X$ represents the ambient space the data is drawn from (typically $\RR^n$) even if the data lives on a submanifold of $X$, and $L$ is a set of labels (often $\{1,\dots,\ell\}$).  Note that points $x\in X$ can be natural or adversarial points.%The following definition complements the definition for adversarial examples by providing a criteria for the local stability of the classifier about a point, which could be an actual test point or an adversarial example: 

\begin{definition}
Let $\CC:X\to L$ be a classifier, $x \in X$, $\gamma\in(0,1)$, and $\sigma>0$. We say $x$ is \emph{$(\gamma,\sigma)$-stable} with respect to $\CC$ if $\mathbb{P}[\CC(x')=\CC(x)] \geq \gamma$ for $x' \sim \rho = N(x, \sigma^2 I)$; i.e. $x'$ is drawn from a Gaussian with variance $\sigma^2$ and mean $x$.
\end{definition}

In the common setting when $X=\RR^n$, we have
\[\mathbb{P}[\CC(x')=\CC(x)] = \int_{\RR^n} \mathbbm{1}_{\CC^{-1}(\CC(x))} (x') d\rho (x') = \rho(\CC^{-1}\CC(x)).\]
Note here that $\CC^{-1}$ denotes preimage. %In the case of images drawn from $\RR^n$, we can write this integral precisely as
One could substitute various probability measures $\rho$ above with mean $x$ and variance $\sigma^2$ to obtain different measures of stability corresponding to different ways of sampling the neighborhood of a point.  Another natural choice would be sampling the uniform measure on balls of changing radius. Based on the concentration of measure for both of these families of measures (see Appendix \ref{sec:concentration}), we do not anticipate significant qualitative differences in these two approaches. We propose Gaussian sampling because it is also a product measure, which makes it easier to sample and simplifies some other calculations below.

For the Gaussian measure, the probability above may be written more concretely as
\begin{equation}\label{EQN:Gaussian}
\frac{1}{\left(\sqrt{2\pi}\sigma\right)^{n}} \int_{\RR^n} \mathbbm{1}_{\CC^{-1}(\CC(x))} (x')e^{-\frac{\norm{x - x'}^2}{2\sigma^2}} dx'.
\end{equation}
In this work, we will conduct experiments in which we estimate this stability for fixed $(\gamma,\sigma)$ pairs via a Monte Carlo sampling, in which case the integral \eqref{EQN:Gaussian} is approximated by taking $N$ i.i.d. samples $x_k \sim \rho$ and computing
\[
    \frac{\norm{x_k : \CC(x_k) = \CC(x)}}{N}.
\]
Note that this quantity converges to the integral \eqref{EQN:Gaussian} as $N\to\infty$ by the Law of Large Numbers.

The ability to adjust the quantity $\gamma$ is important because it is much weaker than a notion of stability that requires a ball that stays away from the decision boundary as in \cite{Khoury2018}. By choosing $\gamma$ closer to $1$, we can require the samples to be more within the same class, and by adjusting $\gamma$ to be smaller we can allow more overlap.

We also propose a related statistic, \emph{persistence}, by fixing a particular $\gamma$ and adjusting $\sigma$. For any $x\in X$ not on the decision boundary, for any choice of $0<\gamma<1$ there exists a $\sigma_\gamma$ small enough such that if $\sigma < \sigma_\gamma$ then $x$ is $(\gamma,\sigma)$-stable. We can now take the largest such $\sigma_\gamma$ to define persistence.

%In our experiments, $\gamma$ is fixed and $\sigma$ is adjusted to determine the largest $\sigma$ for which an image is $(\gamma,\sigma)$-stable.  We define this to be persistence as follows.


\begin{definition}
    Let $\CC:X\to L$ be a classifier, $x \in X$, and $\gamma\in(0,1)$. Let $\sigma_\gamma^*$ be the maximum $\sigma_\gamma$ such that $x$ is $(\gamma, \sigma)$-stable with respect to $\CC$ for all $\sigma<\sigma_\gamma$. We say that $x$ has \emph{$\gamma$-persistence} $\sigma_\gamma^*$.
\end{definition}

The $\gamma$-persistence quantity $\sigma_\gamma^*$ measures the stability of the neighborhood of a given $x$ with respect to the output classification. Small persistence indicates that the classifier is unstable in a small neighborhood of $x$, whereas large persistence indicates stability of the classifier in a small neighborhood of $x$. In the later experiments, we have generally taken $\gamma = 0.7$. This choice is arbitrary and chosen to fit the problems considered here. In our experiments, we did not see significant change in results with small changes in the choice of $\gamma$.

In order to better understand the notion of $\gamma$-persistence, consider a decision boundary that is the boundary of a conical wedge domain $W^n_k \subset \RR^n$, where $0<k\leq n$, defined by 
\[
    W^n_k = \{(x_1, \ldots, x_n) \in \RR^n : x_1 \geq 0, \ldots, x_k \geq 0\}.
\]
One can consider this as a Cartesian product of a half space and a positive orthant (see Figure \ref{fig:orthants} for the three possibilities if $n=3$). The boundary of $W^n_k$ consists of parts of hyperplanes (in fact, $W^m_\ell$ for $m\leq n$ and $\ell \leq k$). It is clear that for larger $k$, there is more curvature (this can be made precise using the notion of curvature measures via tube formulas as in \cite{morvan}). We now explore $\gamma$-persistence for data points inside wedge domains, which will serve as a local model for adversarial examples within their adversarial classes.
%For example, in three dimensions, we can consider decision boundaries shaped like a plane, two planes intersecting orthogonally and meeting along a line, or three planes intersecting orthogonally and all meeting at a point. For a point that is equidistant to the planes, we can compute the persistence exactly as follows.

%Recall the formula (\ref{EQN:Gaussian}).
\begin{proposition} \label{prop:orthants}
    If the point $x \in W^n_k$ such that $W^n_k$ describes the class of $x$ and $x$ is a distance $d$ from each sheet of the boundary of $W^n_k$, then the integral (\ref{EQN:Gaussian}) is equal to
\[
    \left( \frac{1}{2}\left(  1+\operatorname{erf}\left(  \frac{d}{\sqrt
    {2}\sigma}\right)  \right) \right)^k,
\]
    where $\operatorname{erf}(z)=\frac{2}{\sqrt{\pi}}\int_0^z e^{-y^2}dy$ is the error function.
    It follows that the $\gamma$-persistence of $x$ is
\[
    \sigma_\gamma^* = \frac{d}{\sqrt{2}\operatorname{erf}^{-1} \left( 2 \gamma^{1/k} -1\right)}.
\]
\end{proposition}

\begin{proof}
First, consider a decision boundary consisting of a hyperplane in $\RR^n$
and suppose that the point $x$ is a distance $d$ from that decision boundary. If we rotate the situation so that the plane is orthogonal to the $x_{n}$-axis, we can compute the integral \eqref{EQN:Gaussian} exactly:
\begin{align*}
\frac{1}{\left(\sqrt{2\pi}\sigma\right)^{n}}& \int_{-\infty}^{\infty} \cdots \left( \int_{-\infty}^{\infty}\left( \int_{-\infty}^{x_n+d} e^{-\frac{\left(  x'_n-x_n\right)  ^{2}}{2\sigma^2}
}dx'_n \right)e^{-\frac{\left(  x'_{n-1}-x_{n-1}\right)  ^{2}}{2\sigma^2}} dx'_{n-1}\right) \cdots e^{-\frac{\left(  x'_{1}-x_{1}\right)  ^{2}}{2\sigma^2}} dx'_{1}
\\
%&=\sqrt{2\sigma}\int_{-\infty}^{d/\sqrt{2\sigma}}e^{-y^{2}}dy\\
&=\frac{1}{2}\left(  1+\operatorname{erf}\left(  \frac{d}{\sqrt
{2}\sigma}\right)  \right).
\end{align*}
Since the Gaussian factorizes, a similar calculation shows that for the point $x$ of distance $d$ away from the sheets of $W_k^n$, the integral \eqref{EQN:Gaussian} is the $k$-th power of the expression above. The fact that this is equal to $\mathbb{P}[\CC(x')=\CC(x)]$ for $x' \sim \rho = N(x, \sigma^2 I)$ completes the proof.
%a point $x$ that is $d$ distance away from $k$ planes that make up a convex cone, the integral is the $k$-th power of the expression above.
% \[
%     \left( \frac{1}{2}\left(  1+\operatorname{erf}\left(  \frac{d}{\sqrt
% {2}\sigma}\right)  \right) \right)^k.
% \]
\end{proof}


Note that these results are independent of the ambient dimension ($n$) and only depend on the number of hyperplanes ($k$) making up the cone piece. This fact is related to a similar observation about the Gaussian isoperimetric inequality (e.g., \cite{ledoux1996isoperimetry}).

\begin{figure}[ht]
    \centering
    \begin{tikzpicture}[tdplot_main_coords, scale = 2]
 
 % Create a point (P)
 \coordinate (P) at ({1/sqrt(3)},{1/sqrt(3)},{1/sqrt(3)});
 
 
 %\draw[dashed, gray] (0,0,0) -- (-1,0,0);
 %\draw[dashed, gray] (0,0,0) -- (0,-1,0);
 
 % Axes in 3 d coordinate system
 %\draw[-stealth] (-1,0,0) -- (1.80,0,0);
 %\draw[-stealth] (0,-1,0) -- (0,1.30,0);
 %\draw[-stealth] (0,0,0) -- (0,0,1.30);
 \draw plot [mark=*,mark size=.3](P) ;
 % Line from the origin to (P)
 %\draw[thick, -stealth] (0,0,0) -- (P);
 
 \filldraw[
 draw=red,%
 fill=red!20,%
 ]          (0,0,0)
 -- (1,0,0)
 -- (1,0,1)
 -- (0,0,1)
 -- cycle;
 
%  \filldraw[
% draw=red,%
% fill=red!20,%
% ]          (0,0,0)
% -- (-1,0,0)
% -- (-1,0,1)
% -- (0,0,1)
% -- cycle; 
 

% Projection of the point XZ plane
%\draw[thin, dashed] (P) --++ (0,0,{-1/sqrt(3)});
\draw[thin, dashed] (P) --++ (0,{-1/sqrt(3)},0);
%\draw[thin, dashed] (P) --++ ({-1/sqrt(3)},0,0);
 

\end{tikzpicture}
\hspace{5em}
\begin{tikzpicture}[tdplot_main_coords, scale = 2]

% Create a point (P)
\coordinate (P) at ({1/sqrt(3)},{1/sqrt(3)},{1/sqrt(3)});


% \draw[dashed, gray] (0,0,0) -- (-1,0,0);
% \draw[dashed, gray] (0,0,0) -- (0,-1,0);
% % Axes in 3 d coordinate system
% \draw[-stealth] (-1,0,0) -- (1.80,0,0);
% \draw[-stealth] (0,-1,0) -- (0,1.30,0);
% \draw[-stealth] (0,0,0) -- (0,0,1.30);
% Line from the origin to (P)
%\draw[thick, -stealth] (0,0,0) -- (P);

\filldraw[
draw=red,%
fill=red!20,%
]          (0,0,0)
-- (1,0,0)
-- (1,0,1)
-- (0,0,1)
-- cycle;

\filldraw[
draw=red,%
fill=red!20,%
]          (0,0,0)
-- (0,1,0)
-- (0,1,1)
-- (0,0,1)
-- cycle; 





% Projection of the point on XZ and YZ planes
%\draw[thin, dashed] (P) --++ (0,0,{-1/sqrt(3)});
\draw[thin, dashed] (P) --++
(0,{-1/sqrt(3)},0);
\draw[thin, dashed] (P) --++
({-1/sqrt(3)},0,0);

\draw plot [mark=*,mark size=.3](P) ;

\end{tikzpicture} 
\hspace{5em}
\begin{tikzpicture}[tdplot_main_coords, scale = 2]

% Create a point (P)
\coordinate (P) at ({1/sqrt(3)},{1/sqrt(3)},{1/sqrt(3)});

 
% \draw[dashed, gray] (0,0,0) -- (-1,0,0);
% \draw[dashed, gray] (0,0,0) -- (0,-1,0);
 
 % Axes in 3 d coordinate system
% \draw[-stealth] (-1,0,0) -- (1.80,0,0);
% \draw[-stealth] (0,-1,0) -- (0,1.30,0);
% \draw[-stealth] (0,0,0) -- (0,0,1.30);
 \draw plot [mark=*,mark size=.3](P) ;
 % Line from the origin to (P)
 %\draw[thick, -stealth] (0,0,0) -- (P);
 
 \filldraw[
draw=red,%
fill=red!20,%
]          (0,0,1)
-- (0,1,1)
-- (1,1,1)
-- (1,0,1)
-- cycle; 
 
 \filldraw[
 draw=red,%
 fill=red!20,%
 ]          (0,0,0)
 -- (1,0,0)
 -- (1,0,1)
 -- (0,0,1)
 -- cycle;
 
 \filldraw[
 draw=red,%
 fill=red!20,%
 ]          (0,0,0)
 -- (0,1,0)
 -- (0,1,1)
 -- (0,0,1)
 -- cycle; 



  \draw plot [mark=*,mark size=.3](P) ;

 % Projection of the point on XZ,YZ, XY planes
 \draw[thin, dashed] (P) --++ (0,0,{1/sqrt(3)});
 \draw[thin, dashed] (P) --++
 (0,{-1/sqrt(3)},0);
 \draw[thin, dashed] (P) --++
 ({-1/sqrt(3)},0,0);

 \filldraw[
draw=red,%
fill=red!20,%
opacity=.5]          (0,0,1)
-- (0,1,1)
-- (1,1,1)
-- (1,0,1)
-- cycle; 

\draw[red] (0,1,1) --(1,1,1);
\draw[red] (1,0,1) --(1,1,1);

 
 \end{tikzpicture}

\caption{Views of different decision boundaries from Proposition \ref{prop:orthants} in the case $n=3$ and $k=1$ (left), $k=2$ (center), and $k=3$ (right). The point $x$ of Proposition \ref{prop:orthants} is shown in black, and dashed lines indicate the shortest distances to the boundary.}
\label{fig:orthants}
\end{figure}

Observe from Proposition \ref{prop:orthants} that if the distance $d$ to the decision boundary is fixed, then the more planes that make up the decision boundary, the smaller the persistence will be.  For illustration, Figure \ref{FIG:Persistence} shows the $0.7$-persistence for the point $x$ in Proposition \ref{prop:orthants} as a function of the number of planes $k$ with $d=1$. Observe that when $k=1$, the $0.7$-persistence is approximately $1.91$ despite the distance from the decision boundary being equal to $1$; this is due to the fact that one must sample from a Gaussian with larger variance to have 30\% of the samples be on the other side of a single plane decision boundary.  Additionally, as $k$, and hence curvature of the boundary, increases, the persistence value becomes less than the distance to the nearest decision boundary, which remains $1$. This illustrates that persistence carries more information regarding the landscape of the decision boundary about $x$ than merely the distance to the boundary.  Note also that if the initial point is outside the cone, then the persistence will be significantly larger. This demonstrates how, even if we consider points equally close to the decision boundary, the persistence can distinguish between being in a location that is inside a cone and outside a cone, as well as how sharp the boundary of those cones may be. The existence of such cones or curved decision boundaries is both seen experimentally ~\cite{Fawzi2018empirical,roth19aodds} and theorized ~\cite{shamir2021}. It is expected that adversarial examples lie inside the cone, as modeled by the wedge domains, and the natural examples lie outside the cone or wedge domain.

%It follows that if we fix the distance $d$ to the decision boundary, the more planes making up the decision boundary, the smaller the persistence will be. For instance, in the case of $d=1$ and a single hyperplane decision boundary, the $0.7$-persistence is approximately $1.91$, whereas a two hyperplane decision boundary has $0.7$-persistence of approximately $1.02$ and a three hyperplane decision boundary has $0.7$-persistence of approximately $0.82$. Note that if the initial point is outside the cone, then the persistence will be significantly larger. This demonstrates how, even if we consider points equally close to the decision boundary, the persistence can distinguish between being in a location that is inside a cone and outside a cone, as well as how sharp the boundary of those cones may be. The existence of such cones or curved decision boundaries is both seen experimentally ~\cite{Fawzi2018empirical,roth19aodds} and theorized ~\cite{shamir2021}.

\begin{figure}[h!]
\centering
\includegraphics[width=.4\textwidth]{c2_figures/Persistence.png}
\caption{Plot of $0.7$-persistence vs. $k$ for a point $x$ that is distance 1 from all sheets of the conic domain $W_k^n$, as in Proposition \ref{prop:orthants}.}\label{FIG:Persistence}
\end{figure}


In our experiments, we numerically estimate $\gamma$-persistence via a bisection algorithm that we term the Bracketing Algorithm (Appendix \ref{sec:bracketing}).  Briefly, the algorithm first chooses search space bounds $\sigma_{\min}$ and $\sigma_{\max}$ such that $x$ is  $(\gamma,\sigma_{\min})$-stable but is not $(\gamma,\sigma_{\max})$-stable with respect to $\CC$, and then proceeds to evaluate stability by bisection until an approximation of $\sigma_\gamma^*$ is obtained.


%This is accomplished by a bracketing procedure: we first expand the search space bounds $\sigma_{\min}$ and $\sigma_{\max}$ so that the average number of samples at these bounds are below (respectively above) $\gamma$.  This search space is then sequentially bisected to identify a $\sigma$ corresponding with $\gamma$ (the full algorithm is presented in the Appendix).

%We can compute approximate the $\gamma$-persistence using a bisection algorithm we call the Bracketing Algorithm. The Bracketing Algorithm is given as Algorithm \ref{bracketing} in Appendix \ref{sec:bracketing}.  

%\renewcommand{\baselinestretch}{1.0}

%\renewcommand{\baselinestretch}{1.5}

\section{Experiments} \label{sec:experiments}

%???Did we try Carlini-Wagner method? -- B2 not yet, working on it for Imnet

% B2 -- here's what we have ready to go

In this section we investigate the stability and persistence behavior of natural and adversarial examples for MNIST ~\cite{MNIST} and ImageNet ~\cite{ILSVRC15} using a variety of different classifiers. For each set of image samples generated for a particular dataset, model, and attack protocol, we study $(\gamma,\sigma)$-stability and $\gamma$-persistence of both natural and adversarial images, and also compute persistence along trajectories from natural to adversarial images. In general, we use $\gamma = 0.7$, and note that the observed behavior does not change significantly for small changes in $\gamma$. While most of the adversarial attacks considered here have a clear target class, the measurement of persistence does not require considering a particular candidate class. These experiments were performed using PyTorch on an HPC configured with 28 CPUs, 192gb of memory, and 1 nvidia p100 GPU per node. Total compute time needed to generate the results presented was approximately 300 Teraflop/s-days. 




% Adversarial examples are generated using Iterative Gradient Sign Method (IGSM) ~\cite{kurakin_adversarial_2016}, which is an iterative version of the Fast Gradient Sign Method (FGSM) \cite{goodfellow_explaining_2014}, as well as the more primitive Limited-memory Broyden-Fletcher-Goldfarb-Shanno (L-BFGS) optimization algorithm ~\cite{liu1989limited}. 

% The neighborhoods around datapoints and adversarial examples are sampled using Gaussians with varying standard deviation $\sigma$, and Algorithm \ref{bracketing} is used to approximate $\gamma$-persistence corresponding to $\gamma=0.7$. The resultant $0.7$-persistence $\sigma_{.7}^*$ statistically identifies examples as being $(0.7,\sigma_{.7}^*)$-stable, meaning that 70\% of the samples drawn from a Gaussian with standard deviation $\sigma$ are classified the same as the original class by the model. 

% The first test of the ideas behind $(\gamma, \sigma)$-stability is to consider what happens to Gaussian samples as the standard deviation is increased from zero. To this end, for each choice of $\sigma$ ??Where?? we took 1000 samples around the original image or adversarial image and plotted the count of how many were classified with each label. These results are seen in Figures ???? %Algorithm \ref{bracketing} is used to approximate $\gamma$-persistence corresponding to $\gamma=0.7$. The resultant $0.7$-persistence $\sigma$ statistically identifies examples as being $(0.7,\sigma)$-stable, meaning that 70\% of the samples drawn from a Gaussian with standard deviation $\sigma$ are classified the same as the original class by the model. 
% In order to understand the impact of model complexity on $(\gamma, \sigma)$-stability of adversarial examples, we considered the framework of ~\cite{Szegedy2013}, looking at a variety of networks of differing complexities, including both fully-connected and convolutional neural networks.


\subsection{MNIST Experiments}

%The MNIST dataset consists of 28 by 28 pixels, so it can naturally be considered as a data set on a 784 dimensional vector space. The size of this data makes it ideal for initial testing. 
Since MNIST is relatively small compared to ImageNet, we trained several classifiers with various architectures and complexities and implemented the adversarial attacks directly. Adversarial examples were generated against each of these models using Iterative Gradient Sign Method (IGSM ~\cite{kurakin_adversarial_2016}) and Limited-memory Broyden-Fletcher-Goldfarb-Shanno (L-BFGS ~\cite{liu1989limited}).


 

\subsubsection{Investigation of $(\gamma, \sigma)$-stability on MNIST}\label{sec:mnist}

We begin with a fully connected ReLU network with layers of size 784, 100, 20, and 10 and small regularization $\lambda = 10^{-7}$ which is trained on the standard MNIST training set. We then start with a randomly selected MNIST test image $x_1$ from the \texttt{1}'s class and generate adversarial examples $x_0,x_2,\dots,x_9$ using IGSM for each target class other than \texttt{1}. The neighborhoods around each $x_i$ are examined by generating 1000 i.i.d. samples from $N(x_i,\sigma^2I)$ for each of 100 equally spaced standard deviations $\sigma\in(0,1.6)$. Figure \ref{fgsmo} shows the results of the Gaussian perturbations of a natural example $x_1$ of the class labeled \texttt{1} and the results of Gaussian perturbations of the adversarial example $x_0$ targeted at the class labeled \texttt{0}. We provide other examples of $x_2,\ldots,x_9$ in the supplementary materials. Note that the original image is very stable under perturbation, while the adversarial image is not. 

% \begin{figure}[ht]
% \includegraphics[trim=200 80 100 100, clip, width = .9\textwidth]
% %[trim=200 80 100 100, clip,width=15cm]
% {c2_figures/Image918-O1Anone_varx40.png}
% \caption{Frequency of each class in Gaussian samples with increasing variance around an adversarial image of a $1$ targeted at $0$ generated using IGSM. The adversarial class is shown as a red curve. The natural image class is shown in black. The bottom shows example sample images.}
% \label{fgsmo}
% \end{figure}


% \begin{figure}[ht]
% \includegraphics[trim=200 80 100 100,clip, width = .9\textwidth]
% %[trim=200 80 100 100, clip,width=15cm]
% {c2_figures/Image918-O1A0_varx40.png}
% \caption{Frequency of each class in Gaussian samples with increasing variance around an adversarial image of a $1$ targeted at $0$ generated using IGSM. The adversarial class is shown as a red curve. The natural image class is shown in black. The bottom shows example sample images. }
% \label{fgsma}
% \end{figure}

\begin{figure}[ht]
\includegraphics[width = .49\textwidth]
%[trim=200 80 100 100, clip,width=15cm]
{c2_figures/MNIST1.png} \includegraphics[width = .49\textwidth]
%[trim=200 80 100 100, clip,width=15cm]
{c2_figures/MNIST10.png}
\caption{Frequency of each class in Gaussian samples with increasing variance around a natural image of class \texttt{1} (left) and around an adversarial attack of that image targeted at \texttt{0} generated using IGSM (right). The adversarial class (\texttt{0}) is shown as a red curve. The natural image class (\texttt{1}) is shown in black. Bottoms show example sample images at different standard deviations for natural (left) and adversarial (right) examples.}\label{fgsmo}
\end{figure}



\subsubsection{Persistence of adversarial examples for MNIST}

% For adversarial examples, we are particularly interested in comparing the classification counts around each example relative to the distortion ($\|x\|_2/\sqrt{n}$) introduced to generate the example. We then compute $0.7$-persistence for a variety of models and samples and summarize these results.

To study persistence of adversarial examples on MNIST, we take the same network architecture as in the previous subsection and randomly select 200 MNIST images. For each image, we used IGSM to generate 9 adversarial examples (one for each target class) yielding a total of 1800 adversarial examples. In addition, we randomly sampled 1800 natural MNIST images. For each of the 3600 images, we computed $0.7$-persistence; the results are shown in Figure \ref{fig:IGSMpersistenceMNIST}. One sees that $0.7$-persistence of adversarial examples tends to be significantly smaller than that of natural examples for this classifier, indicating that they are generally less stable than natural images. We will see subsequently that this behavior is typical.

%and generate adversarial examples using IGSM for each of 200 randomly selected MNIST images to each possible target other than the original class (9 total targets) for a total of 1800 adversarial examples. 
 %The images were processed using a bisection algorithm (Algorithm \ref{bracketing} in the supplementary materials) to compute $0.7$-persistence. The results are aggregated in Figure \ref{fig:IGSMpersistenceMNIST}.
\begin{figure}[h!]
\centering
\includegraphics[trim=200 80 100 100, clip,width=.5\textwidth]{c2_figures/original_hist.png}
\caption{Histogram of $0.7$-persistence of IGSM-based adversarial examples (red) and natural examples (blue) on MNIST. %The histogram shows that $0.7$-persistence for adversarial examples tends to be smaller than $0.7$-persistence for natural examples.
}
%\label{fgsmh}
\label{fig:IGSMpersistenceMNIST}
\end{figure}
% TODO : expand figure 13 with a wide sample of adversarial versus natural examples from imagenet. 
%In this experiment, the adversarial examples (red) tended to have a lower $0.7$- persistence than natural images (blue), indicating that they were much less stable than the natural images. %DG: I HAVE REMOVED: We can define a linear classifier on these $\gamma$-persistence values which will identify adversarial attacks with 98\% accuracy. 

%\subsection{Effects of network complexity on persistence}
%{Neighborhood sampling of L-BFGS adversarial examples for MNIST}

Next, we investigate the relationship of network complexity and $(\gamma,\sigma)$-stability by revisiting the now classic work of ~\cite{Szegedy2013} on adversarial examples. 
%In these experiments, we used L-BFGS technique from \cite{Szegedy2013} to prepare adversarial examples. The same network architectures and examples were subjected to $0.7$-persistence analysis to determine the correspondence of stability with network accuracy and average distortion. In this case we will loosely define complexity as the effective number of parameters of a network and distortion is the $\ell^2$ norm divided by square root of the dimension $n$. 
%[??DG??: We need to define complexity and add it to the table]
%\subsubsection{Re-examining Szegedy Results with sampling}
%
Table \ref{table1} recreates and adds on to part of \cite[Table 1]{Szegedy2013} in which networks of differing complexity are trained and attacked using L-BFGS. The table contains new columns showing the average $0.7$-persistence for both natural and adversarial examples for each network, as well as the average distortion for the adversarial examples. The distortion is the $\ell^2$-norm divided by square root of the dimension $n$. The first networks listed are of the form FC10-k, and are fully connected single layer ReLU networks that map each input vector $x \in \RR^{784}$ to an output vector $y \in \RR^{10}$ with a regularization added to the objective function of the form $\lambda\Norm{w}_2/N$, where $\lambda = 10^{-k}$ and $N$ is the number of parameters in the weight vector $w$ defining the network. The higher values of $\lambda$ indicate more regularization.  
%added as regularization to the objective function during training. FC10-2 is the same except with $\lambda = 10^{-2}$ and FC10-0 has $\lambda=1$ (a very large coefficient for regularization). 
FC100-100-10 and FC200-200-10 are networks with 2 hidden layers (with 100 and 200 nodes, respectively) with regularization added for each layer of perceptrons with the $\lambda$ for each layer equal to $10^{-5}, 10^{-5}$, and  $10^{-6}$. Training for these networks was conducted with a fixed number of epochs (typically 21). For the bottom half of Table \ref{table1}, we also considered networks with four convolutional layers plus a max-pooling layer connected by ReLU to a fully connected hidden layer with increasing numbers of channels denoted as as ``C-Ch,'' where C reflects that this is a CNN and Ch denotes the number of channels. A more detailed description of these networks can be found in Appendix \ref{appendix:CNNs}.

\begin{table}[ht]
\centering
\caption{Recreation of ~\cite[Table 1]{Szegedy2013} for the MNIST dataset.  For each network, we show Testing Accuracy (in \%), Average Distortion ($\|x\|_2/\sqrt{n}$) of adversarial examples, and new columns show average $0.7$-persistence values for natural (Nat) and adversarial (Adv) images. 300 natural and 300 adversarial examples generated with L-BFGS were used for each aggregation.}
\label{table1}
\begin{tabular}{lllll}
\toprule
Network & Test Acc & Avg Dist & Persist (Nat) & Persist (Adv) \\
\midrule
FC10-4 & 92.09 & 0.123 & 0.93 & 1.68\\
FC10-2 & 90.77 & 0.178 & 1.37 & 4.25\\
FC10-0 & 86.89 & 0.278 & 1.92 & 12.22\\
FC100-100-10 & 97.31 & 0.086 & 0.65 & 0.56 \\
FC200-200-10 & 97.61 & 0.087 & 0.73 & 0.56 \\
\midrule
C-2 & 95.94 & 0.09 & 3.33 & 0.027 \\
C-4 & 97.36 & 0.12 & 0.35 & 0.027 \\
C-8 & 98.50 & 0.11 & 0.43  & 0.0517 \\
C-16 & 98.90 & 0.11 & 0.53 & 0.0994 \\
C-32 & 98.96 & 0.11 & 0.78 & 0.0836 \\
C-64 & 99.00 & 0.10 & 0.81 & 0.0865 \\
C-128 & 99.17 & 0.11 & 0.77 & 0.0883 \\
C-256 & 99.09 & 0.11  & 0.83 & 0.0900 \\
C-512 & 99.22 & 0.10 & 0.793 & 0.0929 \\
%C-128-2000 & 99.07 & 0.11 & 89.27 & 0.731 & 0.136 \\
%C-128-4000 & 99.13 & 0.098 & 89.71 & 1.024 & 0.424 \\
%C-128-4500 & 99.32 & 0.096 & 90.59 & NA & 0.103 \\
%C-128-4700 & 97.48 & 0.079 & 87.16 & NA & NA \\
%C-128-4708 & 95.69 & 0.077 & 80.90 & 0.15 & 0.0307 \\
%C-128-4712 & 93.04 & 0.135 & 57.11 & 0.14 & 0.0296 \\
%C-128-4714 & 78.87 & 0.211 & 41.61 & 0.059 & 0.012 \\
%C-128-4715 & 65.99 & 0.831 & 23.61 & NA & 0.0092 \\ \hline
\bottomrule
\end{tabular}
\end{table}

The main observation from Table \ref{table1} is that for higher complexity networks,
adversarial examples tend to have smaller persistence than natural examples. Histograms reflecting these observations can be found in the supplemental material. %This can be seen as well in Figure \ref{fig:FC200-200-10}, which shows the $0.7$-persistence for natural and adversarial examples for the network FC200-200-10. 
Another notable takeaway is that for models with fewer effective parameters, the attack distortion necessary to generate a successful attack is so great that the resulting image is often more stable than a natural image under that model, as seen particularly in the FC10 networks. Once there are sufficiently many parameters available in the neural network, we found that both the average distortion of the adversarial examples and the average $0.7$-persistence of the adversarial examples tended to be smaller. This observation is consistent with the idea that networks with more parameters are more likely to exhibit decision boundaries with more curvature.

% \begin{figure}[h!]
% \centering
% \includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/FC200-200-10-distortion_hist.png}\includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/FC200-200-10-gamma1_hist.png}

% \caption{Average distortion for adversarial examples (left) and $0.7$-persistence (right) for FC200-200-10 in Table \ref{table1}}
% \label{fig:FC200-200-10}
% \end{figure}

%B^2 -- we're not using state of the art classifiers... used pre-trained classifiers in order to capture state-of-the-art methods. In particular, we

\subsection{Results on ImageNet}

% For ImageNet, various pretrained networks (vgg16, alexnet, resnet18, densenet161, and squeezenet) were downloaded using torchvision and were attacked with a variety of attack methods %(PGD, FGSM, APGD, CW, ??) 
% using the torchattacks package \cite{kim2021torchattacks}. In all of our tests, we begin with a subset of validation images from the given dataset and generate a collection of adversarial attacks based on those images for each combination of model and attack protocol. 

For ImageNet ~\cite{Imagenet-old}, we used pre-trained ImageNet classification models, including alexnet \cite{alexnet} and vgg16 \cite{simonyan2014very}.
%, resnet18, squeezenet, and densenet161 \cite{}
We then generated attacks based on the ILSVRC 2015 ~\cite{ILSVRC15} validation images for each of these networks using a variety of modern attack protocols, including Fast Gradient Sign Method (FGSM ~\cite{goodfellow_explaining_2014}), Momentum Iterative FGSM (MIFGSM ~\cite{dongMIFGSM}), Basic Iterative Method (BIM ~\cite{kurakin_adversarial_2016}), Projected Gradient Descent (PGD ~\cite{madry_towards_2017}), Randomized FGSM (R+FGSM ~\cite{tramer2018ensemble}), and Carlini-Wagner (CW ~\cite{carlini_towards_2016}). These were all generated using the TorchAttacks \cite{kim2021torchattacks} toolset.
%We first directly examine neighborhood classification counts as with MNIST and observe a similar dichotomy between original and attacked images. 

\subsubsection{Investigation of $(\gamma, \sigma)$-stability on ImageNet}

In this section, we show the results of Gaussian neighborhood sampling in ImageNet. Figures \ref{fig:imagenet_adv} and \ref{fig:persistent_interpimage} arise from vgg16 and adversarial examples created with BIM; results for other networks and attack strategies are similar, with additional figures in the supplementary material. Figure \ref{fig:imagenet_adv} (left) begins with an image $x$ with label \texttt{goldfinch}. For each equally spaced $\sigma\in(0,2)$, 100 i.i.d. samples were drawn from the Gaussian distribution $N(x,\sigma^2I)$, and the counts of the vgg16 classification for each label are shown. In Figure \ref{fig:imagenet_adv} (right), we see the same plot, but for an adversarial example targeted at the class \texttt{indigo\_bunting}, which is another type of bird, using the BIM attack protocol. %There are similar results with other attack protocols, as described in the supplementary materials.

The key observation in Figure \ref{fig:imagenet_adv} is that the frequency of the class of the adversarial example (\texttt{indigo\_bunting}, shown in red) falls off much quicker than the class for the natural example (\texttt{goldfinch}, shown in black). In this particular example, the original class appears again after the adversarial class becomes less prevalent, but only for a short period of $\sigma$, after which other classes begin to dominate. In some examples the original class does not dominate at all after the decline of the adversarial class. The adversarial class almost never dominates for a long period of $\sigma$. 


% \begin{figure}[ht]
% \centering
% \includegraphics[width = .9\textwidth]
% %[trim=200 80 100 100, clip,width=15cm]
% {./c2_figures/ILSVRC2012_val_00001274-vgg16-sampling.png}
% %\caption{Frequency of each class in Gaussian samples with increasing variance around an adversarial image of a $1$ targeted at $0$ generated using IGSM. The adversarial class is shown as a red curve. The natural image class is shown in black. The bottom shows example sample images.}
% \label{fig:imagenet_natural}
% \caption{Frequency of each class in Gaussian samples with increasing variance around a goldfinch image. Bottom shows example sample images. }
% \end{figure}
%
% \begin{figure}[p]
% \centering
% \includegraphics[width = .9\textwidth]
% {./c2_figures/IMNET-class-11-vgg16-RFGSM-48-attack_data-023.png}
% \end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width = .49\textwidth]
%[trim=200 80 100 100, clip,width=15cm]
{./c2_figures/ILSVRC2012_val_00001274-vgg16-sampling.png}
\includegraphics[width = .49\textwidth]
{./c2_figures/IMNET-class-11-vgg16-BIM-48-attack_data-023.png}
%\input{samplot_test.pgf}
\caption{Frequency of each class in Gaussian samples with increasing variance around a \texttt{goldfinch} image (left) and an adversarial example of that image targeted at the \texttt{indigo\_bunting} class and calculated using the BIM attack (right). Bottoms show example sample images at different standard deviations for natural (left) and adversarial (right) examples.}
\label{fig:imagenet_adv}
\end{figure}


\subsubsection{Persistence of adversarial examples on ImageNet}


Figure \ref{fig:persistent_interpimage} shows a plot of the $0.7$-persistence along the straight-line path between a natural example and adversarial example as parametrized between $0$ and $1$. It can be seen that the dropoff of persistence occurs precisely around the decision boundary. This indicates some sort of curvature favoring the class of the natural example, since otherwise the persistence would be roughly the same as the decision boundary is crossed.

\begin{figure}[ht]
\centering
\includegraphics[width = \textwidth]
{c2_figures/persistence_interpolation-IMNET-class-11-vgg16-BIM-48-attack_data-001.png}
\caption{The $0.7$-persistence of images along the straight line path from an image in class \texttt{goldfinch} (11) to an adversarial image generated with BIM in the class \texttt{indigo\_bunting} (14) on a vgg16 classifier. The classification of each image on the straight line is listed as a number so that it is possible to see the transition from one class to another. The vertical axis is $0.7$-persistence and the horizontal axis is progress towards the adversarial image.}\label{fig:persistent_interpimage}
\end{figure}

An aggregation of persistence for many randomly selected images from the \texttt{goldfinch} class in the validation set for Imagenet are presented in Table \ref{TAB:PersistenceAlexVGG}. For each image of a \texttt{goldfinch} and for each network of alexnet and vgg16, attacks were prepared to a variety of 28 randomly selected targets using a BIM, MIFGSM, PGD, FGSM, R+FGSM, and CW attack strategies. The successful attacks were aggregated and their $0.7$-persistences were computed using the Bracketing Algorithm along with the $0.7$-persistences of the original images from which each attack was generated. Each attack strategy had a slightly different mixture of which source image and attack target combinations resulted in successful attacks. The overall rates for each are listed, as well as particular results on the most successful attack strategies in our experiments, BIM, MIFGSM, and PGD. The results indicate that adversarial images generated for these networks (alexnet and vgg16) using these attacks were less persistent, and hence less stable, than natural images for the same models. 


### kill

\begin{table}[ht]
\centering
\caption{The $0.7$-persistence values for natural (Nat) and adversarial (Adv) images along with average distortion for adversarial images of alexnet and vgg16 for attacks generated with BIM, MIFGSM, and PGD on images from class \texttt{goldfinch} targeted toward other classes from the ILSVRC 2015 classification labels.}
\label{TAB:PersistenceAlexVGG}
\begin{tabular}{llll}
\toprule
Network/Method & Avg Dist & Persist (Nat) & Persist (Adv) \\
\midrule
alexnet (total) & 0.0194 & 0.0155 & 0.0049 \\ 
\:\: BIM        & 0.0188 & 0.0162 & 0.0050 \\ 
\:\: MIFGSM     & 0.0240 & 0.0159 & 0.0053 \\ 
\:\: PGD        & 0.0188 & 0.0162 & 0.0050 \\ 
\midrule
vgg16   (total) & 0.0154 & 0.0146 & 0.0011 \\ 
\:\: BIM        & 0.0181 & 0.0145 & 0.0012 \\ 
\:\: MIFGSM     & 0.0238 & 0.0149 & 0.0018 \\ 
\:\: PGD        & 0.0181 & 0.0145 & 0.0012 \\ 
\bottomrule
\end{tabular}
\end{table}

% % figure showing natural image
% \begin{figure}[p]
% \centering
% \includegraphics[width = \textwidth]
% %[trim=200 80 100 10,width = .95\textwidth]
% %trim=200 80 100 100, clip,width=15cm]
% {sampling_histograms/samplot_test.png}
% %{c2_figures/Image918-O1Anone_varx40.png}
% %\input{samplot_test.pgf}
% \caption{Frequency of each class in Gaussian samples with increasing variance around a natural image of a number $1$. The original image class is shown as a black curve. Bottom shows example sample images. }
% \label{fgsmo}
% \end{figure}

% figure showing adversarial image

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% end of what is "written"
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% We first revisit attacks and metrics from ~\cite{Szegedy2013} so that we can compare our stability metric with the properties observed in that original paper. ~\cite{tramer2020adaptive} present methodology and approach necessary to perform adaptive attacks against defended neural networks. These methods provide a framework for our work, which picks a subset of these networks to study in more depth.
% We then further explore the effect of DNN complexity by training, attacking, and analyzing a collection of CNNs of increasing complexity and a collection of CNNs with diminishingly narrower auto-encoders. 

% % B2 -- here's what's coming down the pipeline: 
% Using pre-trained Imagenet classification models (vgg16, alexnet, resnet18, squeezenet, densenet, and inception v3), we generate attacks based on imagenet  ILSVRC 2015 validation images for each of each of these networks \cite{??}. We then generate stability statistics for the original images and adversarial images. 

% % B2 -- here are some things on my todo list but as yet unprioritized
% % option 1 : implement more attacks
% We used the method of ~\cite{carliniwagner} and other typical attacks to generate attacks against each of the MNIST networks mentioned above and also the pretrained Imagenet networks. We generated stability analysis for these attacks as well. 

% % option 2 : generate adaptive attacks against our stability metric when used as a detector
% Working from the Adaptive Adversarial attack framework described by ~\cite{madry_towards_2017}, we wrote a detector based on the stability analysis, attacked this new augmented network (both MNIST and Imagenet). We present the accuracy of our detector model on adversarial images and our rate of detection. In addition, we have performed stability analysis on the resulting attack images and present that as well. 

% % Option 3 : analyze stability of images along the optimization trajectory used to generate the adversarial images 
% [DG: This is not completed, right?] We analyzed stability of images at all steps along the optimization used to generate adversarial attacks to gain insight about how that optimization path corresponds with the decision boundary -- both distortion and persistence are presented along this optimization (plot x-axis is distortion -- plot y-axis is persistence, trajectory is plotted using arrows and dots to show the order of the optimization steps.) (Example images are shown along this path in the adjacent plot)




% We look first at finding adversarial examples of fully connected DNN classifier for MNIST. We then consider adversarial examples of fully connected DNN classifiers for ImageNet. Finally, we explore the influence of the complexity of the DNN by considering both fully connected and convolutional DNNs on MNIST of varying levels of complexity.


% In the following experiments, adversarial examples are generated using Iterative Gradient Sign Method (IGSM) ~\cite{kurakin_adversarial_2016}, which is an iterative version of the Fast Gradient Sign Method (FGSM) \cite{goodfellow_explaining_2014}, as well as the more primitive Limited-memory Broyden-Fletcher-Goldfarb-Shanno (L-BFGS)
% optimization algorithm ~\cite{liu1989limited}. 
% DG: Say more

% \begin{figure}[p]
% %\includegraphics[width=7cm]{c2_figures/Image918-O1A1_varx40.png}
% \includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/Image918-O1A2_varx40.png}\includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/Image918-O1A3_varx40.png}
% \includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/Image918-O1A4_varx40.png}\includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/Image918-O1A5_varx40.png}
% \caption{Frequency of each class in {\it natural} samples with increasing variance around adversarial examples to a $1$ targeted to $2$ (top left), $3$ (top right), $4$ (bottom left), and $5$ (bottom right). The adversarial examples were generated using IGSM. Original Class is shown as a black curve, adversarial in red, all others are blue. 
% Bottom shows example sample images. }
% \label{fgsme}
% \end{figure}

% \begin{figure}[p]
% \includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/Image918-O1A6_varx40.png}\includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/Image918-O1A7_varx40.png}
% \includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/Image918-O1A8_varx40.png}\includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/Image918-O1A9_varx40.png}
% \caption{Frequency of each class in {\it natural} samples with increasing variance around adversarial examples to a $1$ targeted to $6$ (top left), $7$ (top right), $8$ (bottom left), and $9$ (bottom right). The adversarial examples were generated using IGSM. The original class is shown as a black curve, adversarial in red, all others are blue. Bottom shows example sample images. }
% \label{fgsmh}
% \end{figure}


% The neighborhoods around datapoints and adversarial examples are sampled using Gaussians with varying standard deviation $\sigma$, and Algorithm \ref{bracketing} is used to approximate $\gamma$-persistence corresponding to $\gamma=0.7$. The resultant $0.7$-persistence $\sigma$ statistically identifies examples as being $(0.7,\sigma)$-stable, meaning that 70\% of the samples drawn from a Gaussian with standard deviation $\sigma$ are classified the same as the original class by the model. 

% We will consider adversarial examples in the context of two widely used datasets, MNIST digits \cite{MNIST} and ImageNet \cite{Imagenet}.

% % \subsubsection{Gamma-Sigma Stability of FGSM attacks on MNIST}

% % In these initial experiments, the neighborhood around normal and adversarial examples are analyzed via sampling. An image $x$ with classification $\ell$ is selected, adversarial noise $x_a$ is prepared 

% % \begin{figure}[t]
% %   \centering
% % \includegraphics[width=11cm]{c2_figures/O6A9_varx40.png}
% % \includegraphics[width=11cm]{c2_figures/O6A9_varx40_examp.png}
% %   \caption{Top image shows how a regular image, an adversarial image,
% %     and plain noise get classified with added noise indicated on the
% %     $x$-axis. Second image shows in order the Original, IID Gaussian
% %     noise added,  adversarial noise added, and IID Gausian plus
% %     adversarial noise added. }
% % \end{figure}

% % This sampling approach was Each
% % adversarial image in this dataset was bracketted using the sampling
% % technique described above. Within Class 0 of ImageNet (tench/tinca (A
% % type of fish)), 487 samples were processed and of these, 482 met a 5\%
% % threshold, i.e. were less than 95\% of the bracketed additive noise
% % sample distances. This indicates that in exchange for 5\%
% % classification accuracy, we were able to correctly filter out 99.17\%
% % of the adversarial examples. \\




% \subsubsection{$(\gamma, \sigma)$-stability for adversarial examples on ImageNet}
% [??DG?? This section needs picture similar to the previous section] Similar to the above analysis for MNIST, an image $x$ was selected with original class "Rose-Hip," and then an perturbation $x_a$ was found using IGSM so that the sum $x + x_a$ is an adversarial example with class "Baseball." Then 50 Gaussian samples were generated for each of 1000 evenly spaced standard deviation $\sigma$ values. These samples were added to $x$ and $x+x_a$. Figure  \ref{fig:IGSMpersistenceImageNet} shows classifications are colored via a heatmap.

% \begin{figure}[p]
% \includegraphics[width=14cm]{c2_figures/50r1000x_cmap_rand.png}
% \caption{??DG: This is not readable. Heatmaps indicating frequency in each class??? when Gaussian samples are added with given $\sigma$ values. Top starts with a pure black image,
% middle starts with $x$ (the original image), and
% bottom starts with $x + x_a$ (the adversarial image).}
% \label{fig:IGSMpersistenceImageNet}
% \end{figure}

% The $0.7$-persistence of 50 natural examples (DG: of rose hip?) are shown in Figure \ref{fig:IGSMpersistenceImageNet}. In addition, the $0.7$-persistence of the adversarial example is denoted with a red dot. 
% \begin{figure}[p]
% \includegraphics[trim=200 80 100 100, clip,width=12cm]{c2_figures/429-hist.png}
% \caption{Histogram of $0.7$-persistence of ImageNet examples with class "Baseball." ??DG?? Let's replace red dot with something more noticable like an x. Red dot on the left indicates the same $\sigma$ measurement for an adversarial perturbation of a "Rose-Hip" with new class "Baseball" \ref{fgsmhip}} 
% \label{imnetfgsmsamp}
% \end{figure}

% Much like the above case for MNIST, IGSM examples generated on ImageNet were much less $(\gamma,\sigma)$-stable than natural images. DG: Explain:?? 98\% of adversarial images could be distinguished by their $(\gamma,\sigma)$-stability. It should be noted that due to computational intensity of processing ImageNet samples, this dataset is significantly smaller than that used for the MNIST experiments. 

% \subsection{Effects of network complexity on persistence}
% %{Neighborhood sampling of L-BFGS adversarial examples for MNIST}

% As a further study into the relationship of network complexity with $(\gamma,\sigma)$-stability, we revisit the now classic work of \cite{Szegedy2013} on adversarial examples. In these experiments, we used L-BFGS technique from \cite{Szegedy2013} to prepare adversarial examples. The same networks and examples were be subjected to $0.7$-persistence analysis to determine any correspondence of stability with network accuracy and average distortion. 
% [??DG??: We need to define complexity and add it to the table]

% We also consider complexity of this type on convolutional DNNs, consisting of a composition of convolutional layers, followed by a truncation step that drops most of the results from the last convolutional layer, resulting in a low width layer, which is followed by some fully connected layers. 
%In our experiments, 
%a typical network is denoted ``C-Ch-$k$,'' where C reflects that this is a convolutional DNN, Ch denotes the number of channels and $k$ denotes the width of the smallest level, for instance, ``C-128-2''. 
%The ``C'' indicates my convolutional framework. The 128 indicates the number of channels per convolutional layer. The 4714 indicates the number of outputs which are \emph{discarded} from the final layer. In this case, 128 channels in my convolutional structure yields 4716 total output dimensions from the final convolutional layer. Dropping 4714 of these leaves $k = 2$ values which will be passed into the fully connected component of the network. In this way, we can look at more complicated DNNs in the following two dimensions ???
% The network has the form:

% %\vspace{.4cm}

% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
%      Layer & Type & Channels & Kernel & Stride & Output Shape \\
% \hline
%      0 & Image & 1 & NA & NA & $(1, 28, 28)$ \\
%      1 & Conv & 128 & $(5,5)$& $(1,1)$& $(128, 24, 24)$\\
%      2 & Conv & 128 & $(5,5)$& $(1,1)$& $(128, 20, 20)$\\
%      3 & Conv & 128 & $(5,5)$& $(1,1)$& $(128, 16, 16)$\\
%      4 & Conv & 128 & $(5,5)$& $(1,1)$& $(128, 12, 12)$\\
%      5 & Max Pool & 128 & $(2, 2)$ & $(2, 2)$& $(128, 6, 6)$ \\
%      6 & Trunc & 1 & NA & NA & $(k)$ \\
%      7 & FC & $(k, 256)$ & NA & NA & 256 \\
%      8 & FC & $(256, 10)$ & NA & NA & 10 \\
%      \hline
% \end{tabular}

% \noindent Where $k$ is a number of desired output parameters from the convolutional component. 
% [DG: What changes if the number of channels changes? Can we give a general form.]
% We denote such a network as ``C-Ch-$k$,'' where C reflects that this is a convolutional DNN, Ch denotes the number of channels and $k$ denotes the width of the smallest level, for instance, ``C-128-2''.

% %\subsubsection{Re-examining Szegedy Results with sampling}

% Table \ref{table1} is a recreation of \cite[Table 1]{Szegedy2013} in which networks of differing complexity are trained and attacked using L-BFGS. In addition to recreating the results from \cite{Szegedy2013}, the table contains columns for the average $0.7$-persistence natural and adversarial examples for each network. The networks listed are FC10-4, a fully connected network with no hidden layers that that takes the input vector $x \in \RR^{784}$ to an output vector of $y \in \RR^{10}$ with the $\lambda*\Norm{w}_2/N$ where $\lambda = 10^{-4}$ and $N$ is the number of parameters in $w$) added as regularization to the objective function during training. FC10-2 is the same except with $\lambda = 10^{-2}$ and FC10-0 has $\lambda=1$ (a very large coefficient for regularization). FC100-100-10 and FC200-200-10 are networks with 2 hidden layers with regularization added for each layer of perceptrons with the $\lambda$ for each layer equal to $10^{-5}, 10^{-5}$, and  $10^{-6}$. Training for these networks is conducted with a fixed number of epochs. 

% \begin{table}[pt]
% \centering
% \caption{Recreation of ~\cite[Table 1]{Szegedy2013} using pytorch. New columns show average $0.7$-persistence values for adversarial and natural examples. DG: Needs more description??}
% \label{table1}
% \begin{tabular}{llllll}
% \toprule
% Network & Test Acc & Avg Dist & Success Pct & Persist (Nat) & Persist (Adv) \\
% \midrule
% FC10-4 & 92.09 & 0.123 & ?? & 0.93 & 1.68\\
% FC10-2 & 90.77 & 0.178 & ?? & 1.37 & 4.25\\
% FC10-0 & 86.89 & 0.278 & ?? & 1.92 & 12.22\\
% FC100-100-10 & 97.31 & 0.086 & ?? & 0.65 & 0.56 \\
% FC200-200-10 & 97.61 & 0.087 & ?? & 0.73 & 0.56 \\
% \midrule
% C-2-0 & 95.94 & 0.09 & 61.64 & 3.33 & 0.027 \\
% C-4-0 & 97.36 & 0.12 & 81.81 & 0.35 & 0.027 \\
% C-8-0 & 98.50 & 0.11 & 85.47 & NA & 0.0517 \\
% C-16-0 & 98.90 & 0.11 & 88.03 & 0.53 & 0.0994 \\
% C-32-0 & 98.96 & 0.11 & 86.23 & 0.78 & 0.0836 \\
% C-64-0 & 99.00 & 0.10 & 89.74 & 0.81 & 0.0865 \\
% C-128-0 & 99.17 & 0.11 & 87.87 & 0.77 & 0.0883 \\
% C-256-0 & 99.09 & 0.11 & 83.04 & 0.83 & 0.0900 \\
% C-512-0 & 99.22 & 0.10 & 88.88 & 0.793 & 0.0929 \\
% %C-128-2000 & 99.07 & 0.11 & 89.27 & 0.731 & 0.136 \\
% %C-128-4000 & 99.13 & 0.098 & 89.71 & 1.024 & 0.424 \\
% %C-128-4500 & 99.32 & 0.096 & 90.59 & NA & 0.103 \\
% %C-128-4700 & 97.48 & 0.079 & 87.16 & NA & NA \\
% %C-128-4708 & 95.69 & 0.077 & 80.90 & 0.15 & 0.0307 \\
% %C-128-4712 & 93.04 & 0.135 & 57.11 & 0.14 & 0.0296 \\
% %C-128-4714 & 78.87 & 0.211 & 41.61 & 0.059 & 0.012 \\
% %C-128-4715 & 65.99 & 0.831 & 23.61 & NA & 0.0092 \\ \hline
% \bottomrule
% \end{tabular}
% \end{table}
% DG: Why do we need distortion diagram???
% \begin{figure}[p]
% \includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/FC10-4-distortion_hist.png}\includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/FC10-4-gamma1_hist.png}
% \caption{Distortion (left) and $0.7$-persistence (right) for FC-10-4 in Table \ref{table1}}
% \label{table1hist1}
% \end{figure}
% \begin{figure}[pt]
% \includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/FC10-2-distortion_hist.png}\includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/FC10-2-gamma1_hist.png}
% \caption{Distortion (left) and $0.7$-persistence (right) for FC10-2 in Table \ref{table1}}
% \label{table1hist2}
% \end{figure}
% \begin{figure}[p]
% \includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/FC10-0-distortion_hist.png}\includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/FC10-0-gamma1_hist.png}
% \caption{Distortion (left) and $0.7$-persistence (right) for FC10-0 in Table \ref{table1}}
% \label{table1hist3}
% \end{figure}
% \begin{figure}[p]
% \includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/FC100-100-10-distortion_hist.png}\includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/FC100-100-10-gamma1_hist.png}
% \caption{Distortion (left) and $0.7$-persistence (right) for FC100-100-10 in Table \ref{table1}}
% \label{table1hist4}
% \end{figure}
% \begin{figure}[p]
% \includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/FC200-200-10-distortion_hist.png}\includegraphics[trim=200 80 100 100, clip,width=7cm]{c2_figures/FC200-200-10-gamma1_hist.png}
% \caption{Distortion (left) and $0.7$-persistence (right) for FC200-200-10 in Table \ref{table1}}
% \label{table1hist5}
% \end{figure}

%\subsection{CNNs work}

% \section{Conclusion}
% In general, our intuition that adversarial examples are less stable than than natural examples is supported by the results in Table \ref{table1}. 

% The more complex neural networks tended to support less stable adversarial examples, but ones that are closer to the natural examples. 

% Need better discussion and conclusion.
% Key takeaways: 
% 1) Perturbations of adversarial examples do not tend to regress to the original class, but rather to some central class. (Is this still true for Imagenet?)

% Similar to the suggestions of ~\cite{Fawzi2018empirical}, our methods have exploited a notion of curvature based on measures with expanding concentration. A typical example of this method is the tube formulas in integral geometry based on Steiner's early work and greatly generalized to the cases of manifolds, polyhedra, and sets of positive reach \cite{morvan}. These are based on taking uniform measures on balls around the spaces. While this notion is generally considered by taking balls around entire sets, the ideas can also be used to investigate individual points. We consider Gaussian sampling instead because of its ease of use, but the idea that we can change the standard deviations is analogous to changing the radius of uniformly sampled balls. Moreover, concentration inequalities indicate that in high dimensions both cases result in concentration of measure around balls of a radius related to either the standard deviation or radius, respectively (see Section \ref{sec:concentration}). In fact, it may be the case that the differences in the estimates in Proposition \ref{prop:concentration} indicate that Gaussian sampling is, in fact, better than uniform sampling of the ball since the concentration in annuli does not depend on the standard deviation in the case of Gaussian and does depend on radius in the case of uniform.



%, Gaussian measures try to exploit similar structure, but is done in a different way by doing Gaussian sampling about a point instead of approximating curvatures of decision boundaries. Since the results in \cite{Fawzi2018empirical} are based on computing an approximation of a curvature function, they depend on an assumption of being close to the decision boundary. Our method does not need that assumption since the Gaussian sampling is not related to functions but instead based on measures. Curvatures have a close connection to tube formulas \cite{morvan}, which is related to the uniform measure on balls. These measures may not be well-behaved in high dimensions, which is one of the main reasons we choose to instead consider Gaussian measures, which factorize nicely in high dimensions.
%\todo{[DG]: These need to be expanded and placed here or elsewhere, but are extremely important.}



% In these results, we first notice that adversarial attacks generated with IGSM against MNIST are less stable than natural examples from these data sets. This difference is even more pronounced when comparing a adversarial image with other image samples from its target class. This lower stability of adversarial examples is even more pronounced among the attacks prepared via IGSM against VGG16 on ImageNet. Using this technique, we can distinguish adversarial examples prepared by these techniques from natural examples using stability as a test. 

% In the next section of experiments, Table 1 from \cite{Szegedy2013} was reconstructed and augmented with stability measurements. In this table, of the 5 networks trained on the MNIST dataset, the more complicated networks achieved higher accuracy but were defeated by adversarial examples with much less distortion than the simpler adversarial examples. We have added columns indicating the stability of natural and adversarial examples in these models. Adversarial examples generated for more complicated models were much less stable (some less stable than the corresponding natural examples). Adversarial examples generated for the less complicated networks were vastly more stable than natural examples. These results are summarized in the histograms Figure \ref{table1hist1} through \ref{table1hist5}. 

% Type 1: An image whose object measure does not exist under a random
% process $F_w$. This may be recognized in the image space if the
% manifold of measures is observed in the image space. This manifold
% should be of relatively low dimension compared with the dimension of
% the image space, and any images thatvary in directions orthogonal to
% the manifold satisfy Type 1.\\

% \vspace{.3cm}

% e.g. We can consider the image of the
% set of possible handwritten digits under a noiseless
% discretization $A$. It is assumed that the image of the manifold $M$ of
% handwritten digits in $X_O$, $A(M)$ is low dimensional in $X_I$, thus we can 

% \vspace{.3cm}

% consider an $\e$-triangulation of this manifold under $A$ with $\e$
% the resolution of $A$. A type 1 adversarial image will
% be identified as any image that varies more than $\e$ from the
% simplices connecting the triangulation of $A(M)$. 

% Type 2: A perturbation of an image that is indistinguishable under the
% imaging operation (or stochastic imaging process) from an image of an
% admissible object.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%(2)

% \section{Conclusion/Ongoing Work (incorporate in previous)}
% Through the work of Szegedy et al, it was discovered that more sophisticated DNNs can be fooled with smaller adversarial perturbations than less sophisticated DNNs. This speaks to a trade-off between robustness and accuracy which has continued to be an active area of research \cite{tsipras2018robustness}. In this work, we investigated this further by examining neighborhoods around adversarial and natural examples using sampling and $(\gamma,\sigma)$ stability analysis. The same trade-off was observed and we note that highly sophisticated networks admit adversarial examples with very small distortion which can often be identified by a sampling technique. We conclude that such subtle adversarial examples are often not $(\gamma,\sigma)$ stable. One direction for future work is the combination of this sampling method for analyzing neighborhoods with recent geometric interpretations of neural networks. It is theorized that most imaging datasets are samples of low-dimensional manifolds embedded in much higher dimensional representation spaces \cite{Chang2017}. By sampling neighborhoods, we can identify these manifolds and potentially train neural networks which are better restricted to them.  

% Continuing research will focus on understanding the trade-off between the sophistication (corresponding with accuracy) and the distortion and stability of adversarial examples that can be generated. Further numerical experiments can be focused on exploring the geometric properties of trained DNNs. We have observed in this report that the average distortion of examples which achieve a new adversarial class vary non-linearly among different natural images and different network structures. Investigating $(\gamma,\sigma)$ stability of points on paths between natural and adversarial examples or between different natural images may provide more insight into the geometric interpretation of classification boundaries under DNN models. In addition, there are many more adversarial attack types that can be subjected to this analysis.  We have seen that some robust networks only admit adversarial examples with very significant distortion, while other networks admit examples with much smaller distortion. In particular, there is the outstanding question of extending a definition for adversarial examples which emphasizes the subtlety of such examples. 

% Some recent work on this subject has distinguished "fooling" examples which are images that look nothing like the training \cite{nguyen2015deep}. In their work, Nguyen et al. were able to reliably identify such examples through the use of Generative Adversarial Network discriminators. One interesting experiment would be to test GAN discriminators on adversarial examples with varying distortion. If GANs can distinguish adversarial examples with high distortion, while examples with low distortion are less $(\gamma,\sigma)$ stable than natural images, this may establish a no-free-lunch classification of Adversarial Examples. Such classification would have broad implications across the field of machine-learning. 



%Kevin Lin, Mingwei
%Grant funding: BB/DG/KH/CS NSF CCF 1740858 
%Grant funding: BB/DG: NSF DMS 1937229
%Grant funding: DG: NSF DMS 1760538



==> FrontBackMatter/Abbvreviations.tex <==
% Abbvreviations
% Follow the format below to add additional symbols here in the two column table
%
\newcommand{\tb}{\textbf}

\begin{abbreviations}{ll} % Include a list of abbreviations (a table of two columns)

\textbf{LAH} & \textbf{L}ist \textbf{A}bbreviations \textbf{H}ere\\
\textbf{WSF} & \textbf{W}hat (it) \textbf{S}tands \textbf{F}or\\
\textbf{ANN} & \textbf{A}rtificial \textbf{N}eural \textbf{N}etwork\\
\tb{NTK} & \tb{N}eural \tb{T}angent \tb{K}ernel\\
\tb{ML} & \tb{M}achine \tb{L}earning\\


\end{abbreviations}



==> FrontBackMatter/Constants.tex <==
% Constants
%


\begin{constants}{lr@{${}={}$}l} % The list of physical constants is a three column table

% The \SI{}{} command is provided by the siunitx package, see its documentation for instructions on how to use it

Speed of Light & $c_{0}$ & \SI{2.99792458e8}{\meter\per\second} (exact)\\
%Constant Name & $Symbol$ & $Constant Value$ with units\\

\end{constants}

==> FrontBackMatter/Symbols.tex <==
% Symbols
%

\begin{symbols}{lll} % Include a list of Symbols (a three column table)

$a$ & distance & \si{\meter} \\
$P$ & power & \si{\watt} (\si{\joule\per\second}) \\
%Symbol & Name & Unit \\

\addlinespace % Gap to separate the Roman symbols from the Greek

$\omega$ & angular frequency & \si{\radian} \\

\end{symbols}
